Generative Adversarial Equilibrium Solvers

We introduce the use of generative adversarial learning to compute equilibria in general game-theoretic settings, specifically the generalized Nash equilibrium (GNE) in pseudo-games, and its specific instantiation as the competitive equilibrium (CE) in Arrow-Debreu competitive economies. Pseudo-games are a generalization of games in which players' actions affect not only the payoffs of other players but also their feasible action spaces. Although the computation of GNE and CE is intractable in the worst-case, i.e., PPAD-hard, in practice, many applications only require solutions with high accuracy in expectation over a distribution of problem instances. We introduce Generative Adversarial Equilibrium Solvers (GAES): a family of generative adversarial neural networks that can learn GNE and CE from only a sample of problem instances. We provide computational and sample complexity bounds, and apply the framework to finding Nash equilibria in normal-form games, CE in Arrow-Debreu competitive economies, and GNE in an environmental economic model of the Kyoto mechanism.

==> Learning Generalized Nash Equilibrium - ICML/abstract.tex <==
\begin{abstract}
  We introduce the use of generative adversarial learning to compute equilibria in general game-theoretic settings, specifically the \emph{generalized Nash equilibrium} (GNE) in \emph{pseudo-games}, and its specific instantiation as the \emph{competitive equilibrium} (CE) in Arrow-Debreu competitive economies. Pseudo-games are a generalization of games in which players' actions affect not only the payoffs of other players but also their feasible action spaces.
  Although the computation of GNE and CE is intractable in the worst-case, i.e., PPAD-hard, in practice, many applications only require solutions with high accuracy in expectation
  over a distribution of problem instances. We introduce {\em Generative Adversarial Equilibrium Solvers} (\nees{}): a family of generative adversarial neural networks that can  learn GNE and CE from only a sample of problem instances. We provide computational and sample complexity bounds, and apply the framework to finding Nash equilibria in normal-form games, CE in Arrow-Debreu competitive economies, and GNE in an environmental economic model of the Kyoto mechanism.
\end{abstract}
%   \if 0
%     The  computation of equilibrium in economic models has been established as a difficult problem of interest since Arrow and Debreu's seminal work introducing pseudo-games as a general model that captures most economic models. Pseudo-games are a generalization of games, in which the actions taken by each player affect not only other players' payoffs but also their action spaces, for which the canonical solution concept is the generalized Nash equilibrium (GNE). 
%     Pseudo-games include as special instances important economic models such as the Arrow-Debreu model of a competitive economy for which the solution concept is the competitive equilibrium (CE). Although the computation of GNE and CE is intractable in the worst-case, in practice, many applications only require an approximate solution in expectation over a distribution of problem instances.
%     % Although, the computation of these equilibria is intractable in the worst-case, there exists many applications which require approximately correct GNE and CE computation in expectation over a distribution of problem instances.
%     To this end, we introduce Generative Adversarial Equilibrium Solvers (\nees{}), a family of generative adversarial neural networks, which can effectively learn GNE and CE only from a sample of problem instances. We provide computational and sample complexity bounds, and demonstrate the capabilities of our network by solving for Nash equilibrium in normal-form games \dcp{i suggest not to mention regular nash}, CE in Arrow-Debreu competitive economies, and GNE in an environmental economic model of the Kyoto mechanism.
%     \fi
\if 0
Pseudo-games are an economically motivated generalization of games, in which the actions taken by each player affect not only other players' payoffs but also their action spaces. The canonical solution concept for pseudo-games is the generalized Nash equilibrium (GNE), an action profile from which no player can improve their payoffs by deviating to an action in the action space determined by the other players' actions. Pseudo-games include as special instance many important economic models such as the Arrow-Debreu model of a competitive economy for which the solution concept by tradition is the competitive equilibrium (CE). Although the computation of GNE and CE is intractable in the worst-case, in practice, many applications only only require an approximate solution in expectation over a distribution of problem instances.
    % Although, the computation of these equilibria is intractable in the worst-case, there exists many applications which require approximately correct GNE and CE computation in expectation over a distribution of problem instances.
    To this end, we introduce Neural Economic Equilibrium Networks (\nees{}), a family of generative adversarial neural networks, which can effectively learn GNE and CE only from a sample of problem instances. We introduce algorithms to train \nees{} and provide a computational and sample complexity analysis. We demonstrate the capabilities of our network by solving for Nash equilibrium in normal-form games, CE in Arrow-Debreu competitive economies, and GNE in an environmentall economic  model of the Kyoto mechanism.
\fi

==> Learning Generalized Nash Equilibrium - ICML/arrow.tex <==


\subsection{Arrow-Debreu Exchange Economies}\label{sec_ap:arrow_debreu}

\paragraph{Additional Preliminaries.} A \mydef{Competitive equilibrium (CE)} is a tuple which consists of allocations $\allocation \in \R_+^{\numgoods \times \numbuyers}$, and prices $\price \in \R_+^\numgoods$ such that 1.~ all traders $\buyer \in \buyers$ maximize utility constrained by their budget: $\allocation[\buyer]^* \in \argmax_{\allocation[\buyer] \in \consumptions[\buyer]: \allocation[\buyer] \cdot \price \leq \consendow[\buyer] \cdot \price} \util[\buyer](\allocation[\buyer])$, 2.~the markets clear and goods that are not demanded are priced at 0, i.e., $ \sum_{\buyer = 1}^{\numagents} \allocation[\buyer]^*  \leq \sum_{\buyer = 1}^{\numagents} \consendow[\buyer]$ and $\price^* \cdot \left( \sum_{\buyer = 1}^{\numagents} \allocation[\buyer]^*  - \sum_{\buyer = 1}^{\numagents} \consendow[\buyer] \right) = 0$.

A \mydef{Scarf economy}, denoted $(\consendow, \valuation)$, is a Leontief exchange economy with 3 buyers and 3 goods, where the valuation $\valuation$ and endowment $\consendow$ matrices are given as follows:
\begin{align}
    &\consendow = \begin{pmatrix}
        1 & 0 & 0 \\
        0 & 1 & 0 \\
        0 & 0 & 1 \\
    \end{pmatrix} 
    &\valuation = \begin{pmatrix}
        0 & 1 & 0 \\
        0 & 0 & 1 \\
        1 & 0 & 0 \\
    \end{pmatrix}  
\end{align}

\paragraph{Related Work.}

Exchange economies can be solved in polynomial-time via t\^atonnement for CES utilties with $\rho \in [0, 1)$ \cite{bei2015tatonnement}. However,  t\^atonnement is not guaranteed to converge beyond these domains. There exists a convex programs to compute CE in linear exchange markets in polynomial time \cite{devanur2016rational}. The computation of CE is PPAD-complete for Leontief \cite{codenotti2006leontief}, piecewise-linear concave, and additively seperable concave \cite{chen2009settling}, and exchange markets \cite{vazirani2011market, chen2009spending}.
The complexity of CES markets for $\rho \in (\infty, 0)$ is unknown
and remains an open question.

% An \mydef{Arrow-Debreu (Exchange) economy model} consists of a finite set of $\numgoods$ goods, and $\numbuyers$ traders (i.e., agents/consumers). Every trader $\buyer \in \buyers$ has a set of possible consumptions $\consumptions[\buyer] \subseteq \mathbb{R}^{\numgoods}$ which is bounded from below, an endowment of goods $\consendow[\buyer] = \left(\consendow[\buyer][1], \dots, \consendow[\buyer][\numgoods] \right) \in \R^\numgoods$, a utility function $\util[\buyer]: \mathbb{R}^{\numgoods } \to \mathbb{R}$. We denote $\consumptions = \bigtimes_{\buyer \in \buyers} \consumptions[\buyer]$, and $\consendow = \left(\consendow[1], \hdots, \consendow[\numbuyers] \right)^T$. An Arrow-Debreu market is denoted by a tuple $(\util, \consumptions, \consendow)$ A \mydef{Competitive equilibrium (CE)} is a tuple which consists of allocations $\allocation \in \R_+^{\numgoods \times \numbuyers}$, and prices $\price \in \R_+^\numgoods$ such that 1.~traders maximize utility: \\$\forall \buyer \in \buyers \ \ \ \allocation[\buyer]^* \in \argmax_{\allocation[\buyer] \in \consumptions[\buyer] : \allocation[\buyer] \cdot \price^* \leq \consendow[\buyer] \cdot \price^*} \util[\buyer](\allocation[\buyer])$ , 2.~the markets clear and goods that are not demanded are priced at 0, i.e., $ \sum_{\buyer = 1}^{\numagents} \allocation[\buyer]^*  \leq \sum_{\buyer = 1}^{\numagents} \consendow[\buyer]$ and $\price^* \cdot \left( \sum_{\buyer = 1}^{\numagents} \allocation[\buyer]^*  - \sum_{\buyer = 1}^{\numagents} \consendow[\buyer] \right) = 0$. Any Arrow-Debreu market can be formulated as a pseudo-game whose set of GNE is equal to the of CE of the original market \cite{arrow-debreu}. This pseudo-game consists of $\numbuyers + 1$ agents who corresponds to the $\numbuyers$ buyers and a seller. The pseudo-game is given by the following optimization problems for the buyers and the seller respectively:
% \begin{align}
%     &\forall \player \in \players, \quad \max_{\allocation[\buyer] \in \consumptions[\buyer]: \allocation[\buyer] \cdot \price \leq \consendow[\buyer] \cdot \price} \util[\buyer](\allocation[\buyer]) & \max_{\price \in \simplex[\numgoods]} \price \cdot \left( \sum_{\buyer \in \buyers} \allocation[\buyer] - \sum_{\buyer \in \buyers} \consendow[\buyer] \right)
% \end{align}

% Let $\valuation[\buyer] \in \R^\numgoods$, $\subsparams \in (-\infty, 1)^\numbuyers$ be a vector of parameters for the utility function of buyer $\buyer \in \buyers$.
% We consider the following utility function classes:
% Linear: $\util[\buyer](\allocation[\buyer]) = \sum_{\good \in \goods} \valuation[\buyer][\good] \allocation[\buyer][\good]$,  Cobb-Douglas:  $\util[\buyer](\allocation[\buyer]) = \prod_{\good \in \goods} \allocation[\buyer][\good]^{\valuation[\buyer][\good]}$, Leontief:  $\util[\buyer](\allocation[\buyer]) = \min_{\good \in \goods} \left\{ \frac{\allocation[\buyer][\good]}{\valuation[\buyer][\good]}\right\}$, Constant Elasticity of Substitution (CES): $\util[\buyer](\allocation[\buyer]) = \left(\sum_{\good \in \goods} \valuation[\buyer][\good] \allocation[\buyer][\good]^\rho\right)^{\nicefrac{1}{\rho}}$. We note that when we take $\rho = 1$, $\rho \to 0$, and $\rho \to -\infty$ respectively for CES utilities, we obtain linear, Cobb-Douglas, and Leontief utilities.

\paragraph{Experimental Setup.}

We consider experiments on six different exchange economies, each 
with 3 buyers and 5 goods,
and with each economy defined by the utility functions of the players: 1) linear, 2) Cobb-Douglas, 3) Leontief, 4) gross substitutes CES where for all buyers $
\buyer \in \buyers$, $\rho_\buyer \in [0.5, 1]$, 5) gross complements CES where for all buyers $ \buyer \in \buyers$, $\rho_\buyer \in [-1.25, -0.75]$, and 6) mixed CES markets where for all buyers $ \buyer \in \buyers$, $\rho_\buyer \in [-1.25, -0.75] \cap  [0.5, 1]$.\footnote{We reduce the range of the $\rho$ parameter to avoid numerical instability in the computation of utilities.} In addition to these settings, we also consider a Leontief economy with 3 buyers and 3 goods with the goal of solving Scarf economies.


\paragraph{Baselines.} 

We benchmark our algorithm to the most well-known algorithm to solve Arrow-Debreu markets, \mydef{t\^atonnement}, which is an auction-like algorithm that is guaranteed to converge for $\rho \in (1, 0]$ \cite{bei2015tatonnement}, and thus including the Cobb-Douglas cases, and 
the \mydef{exploitability descent} algorithm\footnote{This algorithm simply corresponds to running gradient descent on the exploitability. More information on this algorithm can be found in \citeauthor{goktas2022exploitability} \cite{goktas2022exploitability}.}. %
%
T\^atonnement is defined by the following sequence of prices:
\begin{align}
    \price[][\iter+1] = \price[][\iter] + \eta \sqrt{t} \left( \sum_{\buyer \in \buyers} \allocation[\buyer][][\iter] - \sum_{\buyer \in \buyers} \consendow[\buyer]^{(\iter)} \right) && t = 0, 1, \hdots\\
    \allocation[\buyer][][\iter] \in \argmax_{\allocation[\buyer]: \allocation[\buyer] \cdot \price[][\iter] \leq \consendow[\buyer] \cdot \price[][\iter]} \util[\buyer](\allocation[\buyer]) && \buyer \in \buyers, t = 0, 1, \hdots, 
\end{align}
\noindent while exploitability descent is defined by the following sequence of prices:
\begin{align}
    (\price[][\iter+1], \allocation[][][\iter+1])  = (\price[][\iter], \allocation[][][\iter]) - \eta \sqrt{t} \left(\grad \exploit(\price[][\iter], \allocation[][][\iter]) \right) && t = 0, 1, \hdots 
\end{align}
\noindent where $\exploit(\price[][\iter], \allocation[][][\iter])$ is the exploitability associated with the exchange economy pseudo-game.
For both of these baselines, we use a decreasing learning rate of $\eta \sqrt{t}$ as a function of the number of iterations $t$,
and run the baselines until convergences is observed (we observe that experiments all converge in less than $\leq 200$ iterations). 
%
We note that the use of a learning rate schedule is necessary 
for these algorithms to converge \cite{goktas2022exploitability}.
We run an extensive grid search for $\eta$ over the set \{1.0, 0.5, 0.1, 0.05, 0.01, 0.005, 0.001, 0.0005, 0.0001]\}, selecting $\eta$ to minimize exploitability over the validation set.
We then evaluate these baselines on the test set  with the selected hyperparameters.

\paragraph{Economy Generation.}

For all experiments, we generate 5,000 exchange economy instances,
and set aside 500 markets for each of validation and test.
To generate a market instance, for all buyers $\buyer \in \buyers$ and goods $\good \in \goods$, we sample  each endowment $\consendow[\buyer][\good] \sim \mathrm{Unif}[10^{-9}, 1]$, valuations $\valuation[\buyer][\good] \sim \mathrm{Unif}[10^{-9}, 1]$, and when appropriate
we sample the substitution parameters $\bm{\rho}$ from the  ranges mentioned above. 
A competitive equilibrium is guaranteed to exist 
for exchange markets in all the exchange markets we sample
by Arrow-Debreu's first existence theorem \cite{arrow-debreu} since buyers are endowed with a non-zero amount of each good.

\paragraph{Generator Architecture.}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=\linewidth]{architectures/ad_gen.png}
    \caption{Architecture of the generator of \nees{} for exchange economies.}
    \label{fig:ad_gen}
\end{figure}

We summarize our generator's architecture in \Cref{fig:ad_gen}. As a reminder, in this setting, the generator takes as input an exchange economy $(\consendow, \valuation, \bm{\rho})$\footnote{If the economy is not a CES economy $\bm \rho$ is drawn uniformly at random from $[0.25, 0.75]^\numbuyers$.} and outputs equilibrium prices $\hat{\price}$ and allocations $\hat{\allocation}$. We use the same generator architecture in each of our experiments. 
This generator takes as input the economy matrix $(\consendow, \valuation)$, and passes it through two fully connected layers with ReLU activations and 20 and 10 nodes respectively, to obtain a
\mydef{latent buyer representation}.
The valuations $\valuation$, and endowments $\consendow$ are also separately fed through a network with the same architecture. The network for valuations are augmented with a BatchNorm layer with trainable parameters. This gives us a \mydef{latent valuation representation} and a \mydef{latent  endowment representation}. Each latent representation as well as the element-wise product of  the latent valuations
and latent endowments 
are then concatenated and fed through two fully connected layers with 20 and $\numgoods$ (number of goods)
hidden nodes, respectively, followed by ReLU
activations at each layer. This gives us a 
\mydef{latent market representation}. We then pass the matrix $\valuation^T\consendow$, which we call the {\em good graph}, through two fully connected layers, each
with BatchNorm with trainable parameters and ReLU activation.
These layers have 20 and 10 nodes respectively. We refer to the output of this network as the 
{\em latent good graph}.
We then concatenate the flattened,  latent good graph and latent market representations and feed them through three fully connected layers with 40, 20, and $\numgoods$ (number of goods) nodes, respectively. The outputs of the first two layers are passed through ReLU activations, while the last layer is passed through a softmax. The output of this final layer is the generator's predicted prices $\hat{\price}$. 

Given these prices, we then build an {\em allocation coefficient matrix} of dimensions $\numbuyers \times \numgoods$, where the $(i,j)th$ entry is given by $\frac{\consendow[\buyer] \cdot \hat{\price}}{\hat{\price[\good]}}$. We then calculate the budgets $\consendow \hat{\price}$ of the buyers at prices $\hat{\price}$, and feed them through two fully connected layers, with 30 and 20 nodes respectively and ReLU activations, to obtain a {\em latent budget representation}.
%
Define the {\em tiled prices} as $(\hat{\price}, \hdots, \hat{\price})^T \in \R^{\numbuyers \times \numgoods}$, i.e., a matrix whose rows consists of the vector $\hat{\price}$ repeated $\numbuyers$ times so as to obtain ``$\numbuyers$ tiles of prices''.
We concatenate the latent representation of buyers, the tiled prices, the latent endowment representation, the valuations element-wise divided by the tiled prices, the valuations element-wise multiplied by the tiled prices, and the latent budget on the last dimension, i.e., we append each matrix horizontally so as to preserve the number of rows $\numbuyers$. 
We pass the obtained matrix through 3 fully connected layers, with 100, 50, and 20 nodes respectively and ReLU 
activations. Finally, the output of this network is passed through a  fully connected layer with $\numgoods$
nodes and a softmax activation, leaving us with a matrix of dimension $\numplayers \times \numgoods$ whose rows sum up to 1. 
We multiply this matrix element-wise with the allocation coefficient matrix,
which gives us the allocation $\hat{\allocation}$ for the generator. Notice that $\hat{\allocation}$ is budget feasible at price $\hat{\price}$. The total number of parameters of this generator is 20,855.

\paragraph{Discriminator Architectures.}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=\linewidth]{architectures/ad_discrim.png}
    \caption{Architecture of the generator of \nees{} for exchange economies. The latent consumer representation associated with each exchange economy is described in the description of the discriminator.}
    \label{fig:ad_discrim}
\end{figure}

We summarize the architecture of our network in \Cref{fig:ad_discrim}. As a reminder, in this setting, the generator takes as input an exchange economy $(\consendow, \valuation, \bm{\rho})$ as well as an equilibrium $(\hat{\price}, \hat{\allocation})$ and outputs best-responses $(\price^*, \allocation^*)$.
We build different, modular discriminator architectures for
each of the linear, Cobb-Douglas, Leontief, and CES markets. 
These networks take as input the market matrix $(\consendow, \valuation, \bm{\rho})$ and the equilibrium $(\hat{\allocation}, \hat{\price})$ predicted by the generator.
For all four discriminators, the discriminator outputs price $\price^*$ such that $\price[\good]^* = 1$ if $\good \in \argmax_{\good \in \goods} \sum_{\buyer \in \buyers}\left( \hat{\allocation[ ][ ]}_{\buyer\good} - \consendow[\buyer][\good]\right)$ and $\price[\good]^* = 0$ otherwise. In regard to the allocations, we build a modular allocation network, which takes as input a latent representation of each consumer
as a matrix of dimension $\numbuyers \times p$, and outputs
an allocation. It is in this latent representation
that the discriminators for each economy differ. We describe the latent representation associated with different exchange economies below. 
%
%
We first build an \mydef{allocation coefficient matrix}, where the $(i,j)th$ entry is given by $\frac{\consendow[\buyer] \cdot \hat{\price}}{\hat{\price[\good]}}$. We then pass the matrix of latent consumer representations through three fully connected layers with  100, 50, 20 nodes respectively and ReLU activations.   We take this output and pass it through a final fully connected layer with $\numgoods$ (num goods)
nodes and softmax activations to obtain a matrix of dimension $\numplayers \times \numgoods$ whose rows sum up to 1. We multiply this matrix element-wise with the allocation coefficient matrix,
which gives us {\em allocations} $\allocation^*$ that
are budget feasible at prices $\hat{\price}$.

With the main architecture out of the way, we can now present the 
different latent consumer representations that we
use. For the linear and Cobb-Douglas markets,
the latent representation is simply the matrix that
is given by the valuations matrix $\valuation$ whose rows are divided by $\hat{\price}$. 
For Leontief, the latent representation is the matrix whose $(i,j)th$ entries are given as $\frac{\valuation[\buyer][\good]}{\sum_{\good \in \goods} \price[\good] \valuation[\buyer][\good]}$. Finally, for CES, the latent representation is given as follows: First we obtain latent representations of
each of $\rho$, $\hat{\price}$, $(\consendow[\buyer] \bigodot \price)_{\buyer \in \buyers}^T$, and $\valuation$ by passing them through separate but identical, two fully connected BatchNorm layers with ReLU activations, and
20 and 10 nodes respectively. 
The concatenation of all of these latent representations on the last dimension so as to obtain a matrix with $\numbuyers$ rows and 40 columns, where each row is the concatenation of the latent representations for that consumer gives us the \mydef{latent consumer representation}.

The number of parameters for the discriminator for each of the linear and Cobb-Douglas markets is $6,775$, for Leontief is $7,115$,
and for CES is $14,125$. 

\paragraph{Training Hyperparameters.}

We run our algorithm with an initial warm-up of 10,000 iterations for the discriminator. This warm-up procedure follows exactly the inner loop of \Cref{alg:cumul_regret} but instead uses randomly sampled economies, and randomly sampled action profiles. After the warmup, we use only one step of inner loop iteration for running \Cref{alg:cumul_regret} and run the outer loop for 10,000 iterations. Together with the warmup, the small number of inner loop iterations allow us to significantly speed up the training process. The gradient step is provided by  the ADAM algorithm. For the discriminator, we use the same learning rate for the warm-up and regular training. The learning rates used for ADAM in different markets can be found in \Cref{table:ee_learning_rates}. For all other hyperparameters, we use the default settings of ADAM as given in the OPTAX implementation. 
We process the training data in batches of size 200. We found the learning rates for our algorithm by performing grid search on the validation set for all economies. For the Scarf economy the grid search values were sampled from a standard lognormal distribution.
%
\begin{table}[t]
\centering
\begin{tabular}{c|c|c|}
 Economy Type &  Generator &  Discriminator  \\\hline
 Linear & 0.0001 & 0.001   \\\hline
 Cobb-Douglas & 0.0001 & 0.00001\\\hline
 Leontief & 0.00001 &  0.01  \\\hline
 GS CES &  0.00001 &  0.0001  \\\hline
 GC CES & 0.0001 &  0.0001 \\\hline
 Mixed CES & 0.0001 &  0.00001 \\\hline
 Scarf & 0.000003297599624930109 & 0.0000014820835507051155
\end{tabular}
\caption{Learning rates used for ADAM to train \nees{} in different markets. These learning rates are found via grid search on the validation set for all economies.\label{table:ee_learning_rates}}
\end{table}

We present additional results, missing from the main body of the paper, 
in \Cref{fig:arrow_exploit} and 
\Cref{fig:violin_ad_ap}. We see that \nees{} outperforms all baselines in all economies except Gross Substitutes CES economies for which t\^atonnement performs best. This makes sense since for Gross Substitutes CES economies t\^atonnement is guaranteed to converge to a competitive equilibrium. Even the, we note that the performance of \nees{} is remarkable since it achieves a testing normalized exploitability of 0.005, meaning that \nees{} finds an action profile which is closer than 99.95\% of allocations and prices to a competitive equilibrium.

\begin{figure*}[!ht]
  \centering
  \begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\linewidth]{figures/Arrow-Debreu/linear_exploit_CI1.png}
    % \caption{Caption for image 1}
  \end{subfigure}
%   \hspace{0.5cm}
  \begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\linewidth]{figures/Arrow-Debreu/cd_exploit_CI1.png}
    % \caption{Caption for image 2}
  \end{subfigure}
%   \hspace{0.5cm}
  \begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\linewidth]{figures/Arrow-Debreu/leontief_exploit_CI1.png}
    % \caption{Caption for image 3}
  \end{subfigure}
  \begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\linewidth]{figures/Arrow-Debreu/CES_GC_exploit_CI1.png}
    % \caption{Caption for image 4}
  \end{subfigure}
%   \hspace{0.5cm}
  \begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\linewidth]{figures/Arrow-Debreu/CES_GS_exploit_CI1.png}
    % \caption{Caption for image 5}
  \end{subfigure}
%   \hspace{0.5cm}
  \begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\linewidth]{figures/Arrow-Debreu/CES_mixed_exploit_CI1.png}
    % \caption{Caption for image 6}
  \end{subfigure}
  \caption{Training and Testing Exploitability of \nees{} in linear, Cobb-Douglas, Leontief, GS CES, GC CES, and mixed CES economies.
  \label{fig:arrow_exploit}}
\end{figure*}

\begin{figure*}[!ht]
  \centering
%   \hspace{0.5cm}
  \begin{subfigure}{0.45\linewidth}
    \includegraphics[width= \textwidth]{figures/Arrow-Debreu/GS_CES_violin.png}
    % \caption{Caption for image 5}
  \end{subfigure}
%   \hspace{0.5cm}
  \begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\linewidth]{figures/Arrow-Debreu/GC_CES_violin.png}
    % \caption{Caption for image 6}
  \end{subfigure}
  \caption{Distribution of test exploitability on exchange economies/pseudo-games.
  %. For Leontief, exploitability descent is not shown, as it performed much worse than either methods. 
   \nees{} outperforms all baselines on average in all markets, and in distribution in all markets except Cobb-Douglas.
  \label{fig:violin_ad_ap}}
\end{figure*}



==> Learning Generalized Nash Equilibrium - ICML/comments.tex <==
{\color{blue} David Comments:
Fantastic talk. A few things that came to mind as you presented, in case of use for finalising the paper/future talk:
\begin{enumerate}
    \item Motivation: consider more clearly separating "use for analysis/model" and "use for application" (e.g., cloud) 
    \item In explaining the novelty of GNE to an audience for the first time, I think emphasising simultaneity is important else they think "well, doesn't my action affect your action in chess"?
    \item Another answer to "how can players do this" is that they might find an equil over time (of course it needs the game to be modified in some way such that an action is still well defined if outside of the joint space)
    \item GAN approach is also unsupervised, so you might want a more careful phrasing to distinguish approaches
    \item I always want to know what the input representation of a game is into the G and the D, but that's a detail good to avoid for a talk 
    \item **It's super interesting that this is doing better than 'unsupervised' on Nash games (although I also wondered why you weren't converging... are the results worse than for GNE because action space discrete, making it harder?)
    \item **Given the tatonnement results (and your method doing better), reviewers will definitely need to be convinced you've turned tatonnement as well as possible
    \item For the Scarf result: I also wanted to know how the 'unsupervised' method does
    \item When stating the local optimality convergence result, I think you should say "for an affine G and D"
\end{enumerate}

These notes are from a version of the paper I grabbed yesterday morning.  I hope they help as you push onwards. I'm so impressed that you've already created such a mature draft.
\begin{enumerate}
    \item I would lift up a narrative around the use of "differentiable methods" (i.e., neural nets, deep learning) for economics, including the work of Martin Bichler and work on the design side. I think this is the right way to frame the contribution of this paper. Related to this, on p.2 I think it's important to give more texture on Luke's work and Duan et al, and how they relate to this paper. Also, you should state what, if anything, is known about the use of GANS for game solving, and what is there to take from the Daskalakis 'differential games' work that came up in one of our meetings?

    \item To motivate, it would be helpful if the introduction could give examples of pseudo-games that are not Arrow-Debreu but are more general than regular games. At the moment I think you're non AD examples are all games and not pseudo-games. Also, it would be good, for the uninitiated, to explain whether or not pseudo-games are simultaneous move games, and to emphasize that the action space is continuous and solution concepts do not require randomization (and to state what is known about existence). I think it can also be helpful to explain how PGs generalize regular simultaneous-move games, if indeed they do (i.e., does the action become a mixed strategy in a regular simultaneous move game?). That said, and given how central Arrow-Debreu will be in the paper, it might be a good idea to put a concrete example of an AD set-up in the introduction or preliminaries of the paper in order to explain what a pseudo-game is. I remember that a pseudo-game became clear to me when you explained the dependence of budget sets on prices. (edited) 

    \item The intro, before related work, needs a more extended overview of the algorithm (there should also be a figure showing the generator/discriminator structure somewhere in the paper), the theory you have, and the computational results presented in the paper.

    \item I don't quite understand either Ex 2.1 or Ex 2.2. For Ex 2.1, you have actions in R_+, but do you mean R_{>= 0}? (I think $\R_+$ is strictly larger than zero). Is the intuition for the non-Lipschitz the following: if a2=eps>0 then a1 can be very large and positive and utility to 1 is large and positive. But if a2=0 then utility to 1 is zero? Thus, a1=0 has exploitability zero for a2=0 or large exploitability for a2=eps>0? If this is the idea, it's not coming through clearly at the moment. (By the way, in eq (2), I think it's worth being pedantic and writing b1a2-a1a2+(-a1b2-a1a2)). For Ex 2.2, I don't see the potential for non-Lipschitz exploitability in Eq 8 (also, it's better to format Eqn 6 as b1-a1+(b2-a2)).

    \item In any case, I think you can move the examples and detailed discussion non Liptschitz of exploitability, preventing the straightforward Duan et al. style approach to solving for GNEs, to an appendix. I recommend spending time unpacking the math on p.6 and working hard on explaining (1) why this helps with respect to Lipschitz exploitability, and  (2) why it leads to a GAN formulation. The notation in Eq (10) is problematic because you write $\psi^G$ on an action profile on the LHS and $\psi^G$ on an action profile and some new function f on the RHS. Also, f is not explained before it is used (I think it's the 'defeating action' for each player). The text before Obs 2.3 is also confusing (what does it mean to "compute exploitability "ex post" after having computed expected cumulative regret?) Is Obs 2.3 trivial, with the more important work happening leading up to Eqn 18 and then getting towards Eqn 22? Are you burying the most important part? If so, I think I'd drop the detailed exposition of Obs 2.3 and focus on explaining the more important pieces. I think you need to try to clearly explain (1) what it is, if anything, that makes this Lipschitz (e.g., is it the differentiable hypothesis classes you're referring to leading up to (18)), and then (2) why the formulation you end up with cannot be solved via a standard "flat" unsupervised formulation as in something like bottom p.4., but needs to be solved via a GAN style formulation. In explaining the GAN-style formulation, I wonder if this needs more work. I haven't worked much with GANs, but doesn't the generator they usually just take a random input, and the discriminator a generated output and true output? Your generator seems to take a sampled game as input. Might this need more explanation, e.g., with a figure to map to someones' cartoon understanding of a GAN framework? (Lastly, why is it helpful to talk about Stackelberg formulations in this paper, as you do after Eqn 22? Don't you want to stick with explaining how Eq 22 can be approximately solved via a GAN? I feel getting into Stackelberg discussions can cause confusion over solution concepts. If there's some related work point you want to make, then make it in the related work section. In any case, isn't Alg 1 fixing the follower when taking leader gradients? (Line 3) To me. this looks like Nash not Stackelberg.)
    
    \item Assumption 3.1 needs motivation and discussion. What does this require of the game, and what does this require of the GAN formulation? How practical and well motivated is this? I think you're making assumptions about the neural net architectures that will be quite different from those in your computational work? For Assumption 3.7, it's probably worth reminding that it is non-Lipschitz of exploitability you referred to earlier, not of payoff. (I think Assum 3.7 needs to be moved earlier, since it's used in Lemmas 3.3 and 3.4).
    
    \item  For Section 4.1, should this be compared to Duan et al. or Luke's work? It seems that it would be very useful to show how your GAN approach compares to a direct "learn to minimize exploitability" approach, where that latter approach works. 
    
    \item  I'm worried about the comparison with tatonnement. At the moment it seems it's doing about as well or better than NESS. This needs more discussion. Why is NESS actually better? Also, why do you not include tatonnement in Fig 3, and is it concerning that test is worse than train for NESS? Is there anything that this suggests about your training set-up?

    \item The Kyoto section will want more context, e.g., another paragraph to make it more real and tangible, and probably also a simple numerical example to explain the model. It is important that this application feels very clear and well motivated as a way to anchor the methods in the paper.
\end{enumerate}

Smaller points:
\begin{enumerate}
    \item (p1) I don't get the complexity argument: doesn't it apply equally well to your method, which can be considered an "efficient GNE algorithm". Would it be better just to note this is a worst case complexity result? 
    \item I'd like to see the introduction, and certainly the methods section, speak more directly to how the pseudo-game input is accessed via the learning system; i.e., do you have a representation, or is it accessed through certain kinds of calculations that the generator or discriminator need to be able to do about the game? (edited) 
    \item (p2, top) I find the "not technically a game" language confusing. Are you explaining why pseudo-games are outside the class of regular, simultaneous move games? At the moment you seem to suggest that if one player's action depends on another's then it is not a game, but plenty of sequential move games have this property (chess!).
    \item p.2, para four, this "requires solving a concave maximization problem" needs a citation. Also, I would defer most of the comparative references (e.g., "extends the range of models that we can solve") to the related work, where you can be more specific. At the mo,ent you have to say things like "overwhelming majority".
    \item The related work needs at least one paragraph on neural net/differentiable methods for algorithmic economics, and "nearly all" (top p.3) is not precise enough, and we need more on your [32] paper because it sounds at the moment that it can do a lot and currently undercuts what the reader understands about the contribution in the present paper. Also, it references "first order methods" but you earlier said (mid p.2) that they don't work.
    \item It's feels odd to call this a "classical approach." If so, I'd expect it to have been extensively studied and to have citations! I also don't understand the criticism in regard to needing to generate the entire set of GNE. Why wouldn't I just need to generate one GNE as a prediction target (assuming I know how to break ties across multiple equilibria)?
    \item (top p.5) I don't think you need this comment about the expressiveness of the hypothesis class. An unnecessary detour, perhaps.
\end{enumerate}
That's all for now. Hope it helps!

}

==> Learning Generalized Nash Equilibrium - ICML/conclusion.tex <==
\section{Conclusion}
We introduced \nees{}, a GAN that learns mappings from pseudo-games to GNE. \nees{} outperforms existing methods to compute GNE or CE in exchange economies, and solves even pathological examples, i.e., Scarf economies. Our approach extends the use of exploitability-based learning methods from normal-form games to continuous games, exchange markets, and beyond. \nees{} adds to the growing list of differentiable economics methods that aim to provide practitioners with computational tools for the study of economic properties. \nees{} extends
the range of models for which we have  approximate and reliable solvers. 
For instance, existing algorithms only apply to GNE problems that
are  jointly convex, i.e., pseudo-games for which $\actions$ is a convex set, 
and these algorithms are restricted to relaxation methods 
that are not guaranteed to converge in non-jointly convex games. We show that \nees{} can be trained to convergence in pseudo-games under standard assumptions, hence opening the door to solve pseudo-games beyond those that are jointly convex. 
% Future work should aim to improve the design of the network architectures of \nees{}, 
% as well as devise better training algorithms or loss landscapes.
% \nees{} not only allows to approximately and reliably solves economic models but it also extends the range of models which we can approximately solve. For instance, an overwhelming majority of GNE computation algorithms apply only for a subset of problems which are known as jointly convex, i.e., pseudo-games for which $\actions$ is a convex set, and algorithms that can be used in the jointly convex setting are restricted to relaxation methods which are not guaranteed to converge in non-jointly convex games. We show that \nees{} can be trained to convergence in all problem settings where a solution is guaranteed to exist under suitable assumptions.

==> Learning Generalized Nash Equilibrium - ICML/contributions.tex <==
% \textbf{Contributions.}
\subsection{Contributions}
% \gp{Shouldn't the contribution section include the previous paragraph?}
% 

Earlier  approaches~\cite{duan2021pac,marris2022cce} do not extend even to
continuous (non pseudo-)games, since   evaluating the expected exploitability and its gradient over a distribution of pseudo-games requires  solving as many convex programs as examples in the data set. 
Additionally, in pseudo-games, the exploitability is not Lipschitz-continuous, and thus its gradient is unbounded (\Cref{sec_app:examples}), hindering the use of  standard tools to prove sample complexity and convergence bounds, and making training hard due to exploding gradients.
By delegating the task of computing a best-response to a discriminator,   our method circumvents the issue of solving a convex program, yielding a training  problem given by
a min-max optimization problem whose objective is Lipschitz-continuous, for which gradients can be guaranteed to be bounded under standard assumptions on the discriminator and the payoffs of  players.
%
%

Our approach also extends the class of (non pseudo-)games that can be solved through
deep learning methods from normal-form games to simultaneous-move continuous action
games, since  the non-linear program involved in the computation of  exploitability  in 
previous methods makes them  inefficient in application to continuous-action games.
%, opening the doors to solve many pseudo-games, 
%and including those are  not theoretically well-understood.
We  give polynomial-time convergence guarantees for our training algorithm for the special case of affine generators and affine discriminators (\Cref{thm:convergence_stationary_approx}, \Cref{sec:theory}) and provide generalization bounds for arbitrary function approximators (\Cref{thm:sample_complexity}, \Cref{sec:theory}). Finally, we provide empirical evidence that \nees{} outperforms state of the art baselines in Arrow-Debreu competitive economies, and show that \nees{} can replicate existing qualitative analyses for pseudo-games, suggesting that \nees{} makes predictions that not only have low expected exploitability, but also are qualitatively correct, i.e., close to the true GNE in action space (\Cref{sec:experiments}).

==> Learning Generalized Nash Equilibrium - ICML/experiments.tex <==
\section{Experimental Results}\label{sec:experiments}

We run three sets of experiments, in which we train \nees{} in three different pseudo-game settings.\footnote{We include experiments on normal-form games, as well as all missing additional implementation details in \Cref{sec_app:experiments}.} 
%
% \dcp{suggest to hide the following, and 
% just push all details to appendix, and note in intro that our approach collapses to the existing methods in the case of Nash since we compute exploitability directly}
%
All  experiments are run with 5 randomly selected different seeds, with hyperparameter selection being done over 
all 5 seeds %. Unless otherwise mentioned, all results correspond to an average over these 5 seeds, with
and confidence intervals reported across these seeds as appropriate.

% \textbf{Arrow-Debreu exchange economies.}
\subsection{Arrow-Debreu Exchange Economies}
% 
Our first
set of experiments aim to solve CE in Arrow-Debreu exchange economies \cite{arrow-debreu},
%, an instance of generalized Nash equilbrium in a very well-known pseudo-game which has been shown to be provably hard to solve \cite{daskalakis2009complexity, chen2006settling}.
%For ease and clarity, our experiments focus on a special case of Arrow-Debreu competitive economies\footnote{This is without loss of generality as Arrow-Debreu competitive economies can be reduced to Arrow-Debreu exchange economies in polynomial-time.}, namely 
%
a special case of competitive economies with only consumers.\footnote{This is without loss of generality, as Arrow-Debreu competitive economies can be reduced to Arrow-Debreu exchange economies in polynomial-time.}
%
The difficulty in solving the pseudo-game associated with Arrow-Debreu exchange economies---hereafter \mydef{exchange economies}---arises from the fact that it does not fit into any well-defined categories of pseudo-games, e.g., monotone or jointly convex, for which there are  algorithms that converge to GNEs.


An \mydef{exchange economy} $(\util, \consendow)$ consists of a finite set of $\numgoods \in \N_+$ goods and $\numbuyers \in \N_+$ consumers (or traders). Every consumer $\buyer \in \buyers$ has a set of possible consumptions $\consumptions[\buyer] \subseteq \mathbb{R}^{\numgoods}_+$, an endowment of goods $\consendow[\buyer] = \left(\consendow[\buyer][1], \dots, \consendow[\buyer][\numgoods] \right) \in \R^\numgoods$ and a utility function $\util[\buyer]: \mathbb{R}^{\numgoods } \to \mathbb{R}$. We denote 
% $\consumptions = \bigtimes_{\buyer \in \buyers} \consumptions[\buyer]$, and 
$\consendow = \left(\consendow[1], \hdots, \consendow[\numbuyers] \right)^T$. 
Any exchange economy can be formulated as a pseudo-game whose set of GNE is equal to the set of competitive equilibria (CE)\footnote{We refer the reader to \Cref{sec_ap:arrow_debreu} for a definition.} 
of the original economy \cite{arrow-debreu}. This pseudo-game consists of $\numbuyers + 1$ agents, who correspond to the $\numbuyers$ buyers and a seller.
The pseudo-game is given by the following optimization problem, for each buyer $\buyer \in \buyers$, and the seller, respectively:
\begin{align*}
    \!\!\max_{\allocation[\buyer] \in \consumptions[\buyer]: \allocation[\buyer] \cdot \price \leq \consendow[\buyer] \cdot \price} \!\! \util[\buyer](\allocation[\buyer]) \quad \vline \quad \max_{\price \in \simplex[\numgoods]} \price \cdot \!\!\left( \sum_{\buyer \in \buyers} \allocation[\buyer] - \!\!\sum_{\buyer \in \buyers} \consendow[\buyer] \!\!\right).
\end{align*}
% 
Let $\valuation[\buyer] \in \R^\numgoods_+$, $\subsparams \in (-\infty, 1]^\numbuyers$, be a vector of parameters for the utility function of buyer $\buyer \in \buyers$.
In our experiments, we consider the following utility function classes:
\mydef{Linear}: $\util[\buyer](\allocation[\buyer]) = \sum_{\good \in \goods} \valuation[\buyer][\good] \allocation[\buyer][\good]$,  \mydef{Cobb-Douglas}:  $\util[\buyer](\allocation[\buyer]) = \prod_{\good \in \goods} \allocation[\buyer][\good]^{\valuation[\buyer][\good]}$, \mydef{Leontief}:  $\util[\buyer](\allocation[\buyer]) = \min_{\good \in \goods} \left\{ \frac{\allocation[\buyer][\good]}{\valuation[\buyer][\good]}\right\}$, and 
\mydef{constant elasticity of substitution (CES)}: $\util[\buyer](\allocation[\buyer]) = \left(\sum_{\good \in \goods} \valuation[\buyer][\good] \allocation[\buyer][\good]^\rho\right)^{\nicefrac{1}{\rho}}$.  When we take $\rho = 1$, $\rho \to 0$, and $\rho \to -\infty$ for CES utilities, we obtain linear, Cobb-Douglas, and Leontief utilities respectively. We denote $\valuation = (\valuation[1], \hdots, \valuation[\numbuyers])^T$. As is standard in the literature~\cite{fisher-tatonnement, branzei2021proportional}, we assume that for all buyers $\buyer \in \buyers$, $\consumptions[\buyer] = \R_+^\numgoods$. Once a utility function class is fixed, an exchange economy is referred to with the name of the utility function, and can be sampled as a tuple $(\valuation, \consendow) \in \R^{\numbuyers \times \numgoods} \times \R^{\numbuyers \times \numgoods}$ for linear, Cobb-Douglas, and Leontief exchange economies, and as a tuple $(\valuation, \bm{\rho}, \consendow) \in \R^{\numbuyers \times \numgoods} \times \R^{\numbuyers} \times \R^{\numbuyers \times \numgoods}$ for CES exchange economies. For CES exchange economies, 
 we have a \mydef{gross substitute (GS)} and \mydef{gross complements (GC)} CES economy,
 either when $\rho_\buyer \geq 0$ for all buyers 
or  $\rho_\buyer < 0$  for all buyers,  respectively.  Otherwise, this is a
mixed CES economy.

% \textbf{Baselines.}
\paragraph{Baselines}
For  special cases of exchange economies, the computation of CE is well-studied (e.g., \citet{bei2015tatonnement}), allowing us to compare the performance of  \nees{} to known specialized methods.
%, and see how far beyond known domains our method can perform well.
We benchmark \nees{} to \mydef{t\^atonnement} \cite{walras}, which is
an auction-like algorithm that is guaranteed to converge for CES utilities with $\bm{\rho} \in [0, 1)^\numplayers$ \cite{bei2015tatonnement}, including Cobb-Douglas and excluding Linear utilities. We also
benchmark to  \mydef{exploitability descent (or Augmented Descent Ascent)} \cite{goktas2022exploitability}. For each 
of these baselines, we run an extensive grid search over  decreasing learning rates during validation 
(see \Cref{sec_ap:arrow_debreu}). Each baseline was run to convergence.

We report the results of two experiments. First, we 
run our algorithms in linear, Cobb-Douglas, Leontief, GS CES, GC CES, and mixed CES exchange economies (we defer the
results from the GS CES, and  GC CES experiments to the Appendix). We report the distribution of the
exploitability on the test set for \nees{} and the baselines in \Cref{fig:violin_ad} (additional plots can be found in \Cref{sec_ap:arrow_debreu}). 
%
We measure  performance 
w.r.t. the \mydef{normalized exploitability},
which is  the exploitability of the method divided by the average exploitability over the action space. 
We observe that in all economies, \nees{} outputs an action profile that is on average better than at least $99\%$ of the action profiles in terms of exploitability. 
In all four markets, \nees{} on average achieves lower exploitability than the baselines (see \Cref{fig:arrow_exploit}, \Cref{sec_ap:arrow_debreu}). 
We also see in \Cref{fig:violin_ad} that \nees{} outperforms the baselines, in distribution, in every economy
except Cobb-Douglas. This is not surprising since t\^atonnement is guaranteed to converge in Cobb-Douglas economies \cite{bei2015tatonnement}.
%, which leads to exploitabilities being low for all economies and not just on average.
That said,  t\^atonement does not outperform \nees{} on average, since  t\^atonnement's convergence guarantees hold for different learning rates in each market. 

Second, we compare  \nees{} with the performance of t\^atonnment 
in a pathological and well-know Leontief exchange economy, \mydef{the Scarf economy} \cite{scarf1960instable} (\Cref{fig:scarf_economy}). 
Here, we soft start t\^atonnement with the output of \nees{} with some added uniform noise. This additional noise ensures that the starting point of t\^atonnement is distinct from the output of \nees{}).
We see on Figure \ref{fig:scarf_economy} that the prices generated by t\^atonnement  spiral out and settle into an orbit. 
%
This makes sense as, unlike pure Nash equilibria, GNE and CE are not locally stable \cite{flokas2020no}, meaning that soft-starting the algorithm with the output of \nees{} might be worse than using \nees{} alone.\footnote{An implication is that, whereas  \citet{duan2021pac} observe that neural equilibrium mappings can be used to succesfully soft start known learning dynamics that compute Nash equilibria, this 
does not hold in pseudo-games.} 

The success of \nees{} in Leontief exchange economies as well as the Scarf economy is notable, and suggests that  \nees{} might be smoothing out the loss landscape since for these economies the exploitability is non-differentiable. 
%
% \dcp{drop following?}
% In fact, exploitability descent performs erratically in our experiments as demonstrated by \Cref{fig:violin_ad}. We 
% omit the exploitability descent results from \Cref{fig:arrow_scarf}, since the results were too unstable and obstructing the rest of the figure.
%
\begin{figure*}[t]
  \centering
  \begin{subfigure}{0.52\textwidth}
    \includegraphics[width=\linewidth,trim={0cm 0cm 0.25cm 0.2cm},clip]{figures/Arrow-Debreu/linear_violin.png}
    \caption{Linear economy}
  \end{subfigure}
%   \hspace{0.5cm}
  \begin{subfigure}{0.42\textwidth}
    \includegraphics[width=\linewidth,trim={3.1cm 0cm 2cm 0.75cm},clip]{figures/Arrow-Debreu/cd_violin.png}
    \caption{Cobb-Douglas economy}
  \end{subfigure}
%   \hspace{0.5cm}
  \begin{subfigure}{0.52\textwidth}     
    \includegraphics[width=\linewidth,trim={0cm 0cm 0.3cm 0.2cm},clip]{figures/Arrow-Debreu/leontief_violin_all.jpg}
    \caption{Leontief economy}
  \end{subfigure}
%   \begin{subfigure}{0.3\textwidth}
%     \includegraphics[width=\linewidth]{figures/Arrow-Debreu/CES_GC_exploit_CI1.png}
%     \caption{Caption for image 4}
%   \end{subfigure}
%   \hspace{0.5cm}
%   \begin{subfigure}{0.3\textwidth}
%     \includegraphics[width=\linewidth]{figures/Arrow-Debreu/CES_GS_exploit_CI1.png}
%     \caption{Caption for image 5}
%   \end{subfigure}
%   \hspace{0.5cm}
  \begin{subfigure}{0.42\textwidth}
    \includegraphics[width=\linewidth,trim={3.1cm 0cm 1.6cm 0.75cm},clip]{figures/Arrow-Debreu/CES_mixed_violin.png}
    \caption{Mixed CES economy}
  \end{subfigure}
  \caption{The distribution of test exploitability on pseudo-games.
  %. For Leontief, exploitability descent is not shown, as it performed much worse than either methods. 
   \nees{} outperforms all baselines on average in all markets and in distribution in all markets except Cobb-Douglas.\label{fig:violin_ad} 
%   \dcp{Now we have more space, consider this as a 2x2 figure to make the plots larger}
   }
\end{figure*}
% 
% 
\begin{figure}[!ht]
    \centering
    \includegraphics[width =0.5\linewidth]{figures/Arrow-Debreu/scarf_economy.png}
    \caption{A phase portrait of equilibrium prices in the Scarf Economy.  While the output of \nees{} is close to the equilibrium prices, the final prices outputed by t\^atonnement prices are further than the starting prices. 
    % \sdeni{}{This not implies that competitive equilibria are unstable under t\^atonnement dynamics, additionally, }
    % \gp{Maybe we can expand a bit on this? In what sense is the fact that t\^atonnement prices are further than the starting prices a negative aspect. I think there are two bad things here: First instability, second divergence away from equilibrium prices. Maybe point both of these aspects especially since the page break gives us as plenty of space here. On another note can you try to move both Figs 2 and 3 one page forward?}\deni{I can't distinguish between instability, and divergence from equilibrium prices. Doesn't instability capture also divergence away from equilibrium prices? Btw, I want to add as a reminder note here, that although there exists globally stable alternatives to t\^atonnement, e.g., Smale's method, this method cannot be used in all markets since it requires a unique and diffentiable (marshallian) demand.}
    \label{fig:scarf_economy}}
    \vspace{-1em}
\end{figure}

% \textbf{Kyoto joint implementation mechanism.}
\subsection{Kyoto Joint Implementation Mechanism}
% 
We solve a pseudo-game model of the joint implementation mechanism proposed in the Kyoto protocols~\cite{protocol1997kyoto}. The {\em Kyoto Joint Implementation Mechanism} is a {\em cap-and-trade} mechanism that  bounds each country that signed onto the protocol
to emit anthropogenic gases below a particular emission cap. 
Countries bound by the mechanism can  also invest in green projects in other countries, which in return increases their emission caps. \citet{breton2006game} introduce a model of the Kyoto Joint Implementation Mechanism, using this to predict the impact of the mechanism. The model that the authors propose is partially solvable analytically, that is, one can characterize equilibria qualitatively using comparative statics~\cite{nachbar2002general}, but cannot obtain closed-form solutions for GNE.
Moreover, there is no algorithm that is known to converge to the GNE of this pseudo-game,
since it is not monotone. 

Formally, the \mydef{(Kyoto) Joint Implementation Mechanism} (JI)
consists of $\numcountries \in \N_+$ countries. Each \mydef{country} $\country \in \countries$, can make decisions that result in environmentally damaging anthropogenic \mydef{emissions}, $\emit[\country] \in \R_+$, and can make investments $\invest[\country] \in \R^\numcountries$ to offset their emissions. 
The investments $\invest[\country] \in \R^\numcountries$ that each country $\country \in \countries$ makes in another country $\othercountry \in \countries$ offsets that country's emissions by $\invest[\country][\othercountry] \investrate[\othercountry]$, where this is in proportion to an investment return rate $\gamma_j>0$ for country $j$, with
$\investrate \in \R^\numcountries_+$.
Each country $\country$ has a revenue $\revenue[\country]: \R_+^\numcountries \to \R$, which is a
function of its emissions $\emit[\country]$, a cost function $\cost[\country]: \R^{\numcountries \times \numcountries} \to \R$ that is  a function of all investments,
and a negative externality function, $\damage[\country]: \R^\numcountries \to \R$, 
that is a function of the net emissions of all countries.

Each country $\country$ aims to maximize their surplus, which is equal to their revenue minus the costs of their investments, as well as  the negative externalities caused by emissions constrained by keeping their net emissions under an emission cap, $\emitcap[\country] \in \R_+$. Additionally, for all countries $\country \in \countries$, we require the emission transfer balance to hold, i.e., $\emit[\country] - \sum_{\othercountry \in \countries} \invest[\othercountry][\country] \investrate[\othercountry] \geq 0$, that is no country can transfer more emission reduction than they have. This gives the following optimization problem for each country, $\country \in \countries$:
\begin{align*}
   \!\!\! \max_{(\emit[\country], \invest[\country]) \in \R_+ \times \R_+^{\numcountries}}  &\!\! \revenue[\country](\emit[\player]) \!-\! \cost[\country](\invest) \!-\! \damage[\country]\!\left(\! \left\{\! \emit[\country] \!-\! \sum_{\othercountry \in \countries}\!\invest[\othercountry][\country] \investrate[\country] \!\right\}_\country \right)\\
    & \emit[\country] - \sum_{\othercountry \in \countries} \invest[\country][\othercountry] \investrate[\othercountry] \leq \emitcap[\country]\\
    & \emit[\country] - \investrate[\country] \sum_{\othercountry \in \countries} \invest[\othercountry][\country]  \geq 0 \quad \quad \forall \country  \in \countries
\end{align*}
% 
% 
% 
The literature has traditionally assumed that $\revenue[\country](\emit[\player]; \revrate[\country]) = \emit[\player]\left( \revrate[\player] - \frac{1}{2}\emit[\player] \right)$, $\cost[\country](\invest) = \frac{1}{2} \left( \invest[\country][\country]^2 + \sum_{\othercountry \neq \country} \left[ 
(\invest[\country][\othercountry] + \invest[\othercountry][\othercountry])^2 - \invest[\othercountry][\othercountry]^2 \right] \right)$, and $\damage[\country](\emit - \sum_{\country \in \countries} \invest[\country], \damagerate[\country]) = \damagerate[\country] \sum_{\country \in \countries} (\emit[\country] - \sum_{\othercountry \in \countries} \invest[\country][\othercountry])$.
% giving us the following problem:
% \begin{align}
%     &\max_{(\emit[\country], \invest[\country]) \in \R_+ \times \R_+^{\numcountries}} & \emit[\player]\left( \revrate[\player] - \frac{1}{2}\emit[\player] \right) - \frac{1}{2} \left( \invest[\country][\country]^2 + \sum_{\othercountry 
%     \neq \country \in \countries} \left[ 
%     (\invest[\country][\othercountry] + \invest[\othercountry][\othercountry])^2 - \invest[\othercountry][\othercountry]^2 \right] \right) - \damagerate[\country] \sum_{\country \in \countries} (\emit[\country] -  \sum_{\othercountry \in \countries} \invest[\othercountry][\country] \investrate[\country])\\
%     & &\emit[\country] - \sum_{\othercountry \in \countries} \invest[\country][\othercountry] \investrate[\othercountry] \leq \emitcap[\country]\\
%     & &\emit[\country] - \investrate[\country] \sum_{\othercountry \in \countries} \invest[\othercountry][\country] \geq 0
% \end{align}
Fixing these functional forms, we can  sample $(\revrate, \damagerate, \investrate, \emitcap) \in \R^\numagents_+ \times \R^\numagents \times \R^{\numagents \times \numagents} \times \R^\numagents$ and obtain a representation of the JI mechanism.

We run two different experiments to replicate and extend the analysis of~\citet{breton2006game}. 
We first replicate their qualitative analysis of equilibria (\Cref{fig:phase_kyoto}). \citet{breton2006game} introduce a comparative static analysis, in which they fix all parameters of  JI   except for $\revrate$, and characterize the kinds of GNE  as $\revrate$ varies. In \Cref{fig:phase_kyoto}, the six regions correspond to different kinds of GNE. 
For instance in Region~1, both countries emit strictly less than their emission cap (see Section~4 of \citet{breton2006game}). The parts of the plot that are not shaded correspond to pseudo-games for which GNE are not unique,
and for which equilibria cannot be characterized analytically. We superpose on top of this plot
a set of pseudo-games from an unseen test set, and color each pseudo-game by the color of the region whose condition they fulfill.  

%\deni{Rephrased all of this with the nuemrical precision argument removed. That was a bad argument I think the following makes much more sense!}

We observe that with the exception of Regions~1 and~2a, the structure of the GNE generated by \nees{} 
lines up well with 
the type of GNE. We believe that failure to predict Regions~1 and~2a is
due to  the closeness of the action profiles that fit either of these equilibrium types to other ones.  For instance, \nees{} predicts a GNE of type~4b for pseudo-games in Region~2a but these GNE, although qualitatively different, are very close in action space: the only difference between the two regions is that for the type 2a GNE, one player emits strictly less than its  cap and the other emits exactly its cap, while for the type 4b GNE, both players emit exactly their
emission cap. 
% \dcp{careful with `numerical precision` because I feel you argued we're ok from this viewpoint in the intro... maybe just say the profiles are close, just not qualitatively fitting?}
%
A similar conclusion holds for GNE in Region 3a, as predicted in Region~1.

We also solve the JI pseudo-game for a distribution of JI pseudo-games (\Cref{fig:exploit_kyoto}, \Cref{sec_app:experiments}), and 
these results confirm that the testing normalized exploitability is very low. 
We note that \mydef{normalized exploitability} is given as the exploitability 
divided by the average exploitability over the action space, which means that \nees{} has on average a lower exploitability than $\approx 99.5\%$ of the feasible action profiles. 
This confirms our hypothesis that failure to predict Regions~1 and~2a in \Cref{fig:phase_kyoto} arises from
the proximity between GNE of these types and GNE of types 3a or 4a respectively, since according to exploitability there is very little improvement
left for \nees{}.
% 
% 
\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\linewidth]{figures/kyoto/kyoto_phase_test.png}
    \caption{A  taxonomy of different equilibrium types for various  pseudo-games obtained by fixing all parameters, and varying $\revrate$. The $x$ and $y$ axes represent the revenue parameters $\revrate[1]$, $\revrate[2]$ of the countries. The colored regions (obtained analytically) correspond to different qualitative types of GNE  while the dots correspond to  pseudo-games in the test set colored by the GNE types that were predicted for them by \nees{}. 
    \label{fig:phase_kyoto}}
    \vspace{-2em}
\end{figure}
% \deni{Add new pseudo-game + theorem of correctness etc... }
% We provide a new pseudo-game formulation of Arrow-Debreu economies, whose exploitability is much easier to differentiate. 
% \begin{theorem}
% Consider the Arrow-Debreu economie $(\util, \consumptions, \consendow)$, then any WE $(\allocation^*, \price^*)$, corresponds to a Stackelberg equilibrium strategy of the outer player $(\allocation^*, \price^*)$ in the following convex-concave min-max Stackelberg game:
% \begin{align}
%     \min_{(\allocation, \price) \in \consumptions \times \simplex[\numgoods] : \allocation \price \leq \consendow \price} \max_{(\Y, \q) \in \consumptions \times \simplex[\numgoods] : \Y \price \leq \consendow \price} \left(\q - \price \right)^T \left(  \sum_{\buyer \in \buyers} \allocation[\buyer] - \sum_{\buyer \in \buyers} \consendow[\buyer] \right) + \sum_{\buyer \in \buyers} (\consendow[\buyer] \cdot \price ) \left( \log(\util[\buyer](\y_{\buyer}))  - \log(\util[\buyer](\allocation[\buyer])) \right)
% \end{align}
% \end{theorem}
% \begin{figure*}
%      \centering
%      \begin{subfigure}[b]{0.32\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/linear.png}
%          \caption{Linear Arrow-Debreu Market}
%          \label{fig:linear_ad}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.32\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/cobb_douglas.png}
%          \caption{Cobb-Douglas Arrow-Debreu Market}
%          \label{fig:cd_ad}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.32\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/leontief.png}
%          \caption{Leontief Arrow-Debreu Market}
%          \label{fig:leontief_ad}
%      \end{subfigure}
%         \caption{Convergence of sequential exploitability descent in Arrow-Debreu markets.
%         % for \ref{fig:phase_zero_sum_affine} a game with one action, and 
%         }
%         \label{fig:ad}
% \end{figure*}

==> Learning Generalized Nash Equilibrium - ICML/figures/figure_intro_model.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}
    % Seller box
    \node (seller) [rectangle, minimum width=2cm, minimum height=1cm] {Seller};
    
    % Firms boxes
    \node (firm1) [rectangle, below of=seller, xshift=-1.5cm, minimum width=2cm, minimum height=1cm] {Firm 1};
    \node (firm2) [rectangle, below of=seller, xshift=1.5cm, minimum width=2cm, minimum height=1cm] {Firm 2};
    
    % Consumers boxes
    \node (consumer1) [rectangle, below of=firm1, xshift=-1.5cm, minimum width=2cm, minimum height=1cm] {Consumer 1};
    \node (consumer2) [rectangle, below of=firm1, xshift=1.5cm, minimum width=2cm, minimum height=1cm] {Consumer 2};
    
    % Prices arrows
    \draw [->] (seller) -- (firm1);
    \draw [->] (seller) -- (firm2);
    \draw [->] (seller) -- (consumer1);
    \draw [->] (seller) -- (consumer2);
    
    % Money arrow
    \draw [->, dashed] (consumer1) -- (firm1);
    \draw [->, dashed] (consumer2) -- (firm2);
    
    \end{tikzpicture}
    \caption{Depiction of the Telecommunication Power Allocation Pseudo-Game.}
    \label{fig:my_label}
\end{figure}


==> Learning Generalized Nash Equilibrium - ICML/figures/figure_intro_network.tex <==
\begin{figure}
    \centering
    % Data
    \includegraphics[width=1\linewidth]{figures/intro/gaes_intro_arxiv.png}
    \caption{Summary of the Architecture of \nees{}.\label{fig:network_diagram} }
    \vspace{-1em}
\end{figure}

==> Learning Generalized Nash Equilibrium - ICML/gamut.tex <==
\subsection{Normal-form Games} 

Our first set of experiments aims to explore the impact of the accuracy of the discriminator on the performance of the generator. To this end, we consider normal-form games in which there exists a closed form solution for the discriminator. We observe that with an accurate enough discriminator, \nees{} achieves a performance similar to the neural architecture proposed by  \citet{duan2021pac} when using the same equilibrium mapping architecture for the generator.  

In our experiments, we replicate the setup proposed by \citet{duan2021pac}, and we try to solve five
games from the GAMUT library, namely, Traveller's Dilemma, Bertrand Oligopoly, Grab the Dollar, War of Attrition, and Majority Voting. We give a description of each game, as presented by \citet{duan2021pac}:
%
\begin{itemize}
    \item \mydef{Traveler's dilemma}: Each player simultaneously requests an amount of money and receives the lowest of the requests submitted by all players.
    %
    \item \mydef{Grab the dollar}: A price is up for grabs, and both players have to decide when to grab the price. The action of each player is the chosen times. If both players grab it simultaneously, they will rip the price and receive a low payoff. If one chooses a time earlier than the other, they will receive the high payoff, and the opposing player will receive a payoff between the high and the low.
    %
    \item \mydef{War of attrition}: In this game, both players compete for a single object, and each chooses a time to concede the object to the other player. If both concede at the same time, they share the object. Each player has a valuation of the object, and each player’s utility is decremented at every time step.
    %
    \item \mydef{Bertrand oligopoly}: All players in this game are producing the same item and are expected to set a price at which to sell the item. The player with the lowest price gets all the demand for the item and produces enough items to meet the demand to obtain the corresponding payoff.
    %
    \item \mydef{Majority Voting}: This is an $n$-player symmetric game. All players vote for one of the other players. Players’ utilities for each candidate being declared the winner are arbitrary. If there is a tie, the winner is the candidate with the lowest number. There may be multiple Nash equilibria in this game.
\end{itemize}

\paragraph{Game Generation.}

We use the {\em GAMUT library} \cite{nudelman2004run}, which is a normal-form game generation library designated for testing game-theoretic algorithms, to generate a data set of games. 
Following \citet{duan2021pac}, the games were generated so that payoffs were normalized between $[0,1]$, with all other parameters drawn randomly. We generate 2000 games with 2 players and 300 actions for both players and for each game category, setting aside 200 for validation and 100 for testing. 

\paragraph{Network Architecture.}

In all our experiments, we use a generator for \nees{} that has the same architecture as the equilibrium solver proposed by \citet{duan2021pac}. Namely, we use a neural network with 4 hidden layers each with 1024 nodes and ReLU activations. The final layers of the generator have the same dimension as an action profile and each action in the profile is passed through a player-wise softmax activation.
We augment the entire network with BatchNorm layers with non-trainable parameters after each activation layer. The total number of parameters for this generator is 20,855.


To explore how the accuracy of \nees{}'s generator degrades as one uses more and more approximate discriminators, we consider 4 types of  discriminators: a true discriminator that takes as input every player's expected payoffs for all actions and outputs the action with the highest payoff (this discriminator recovers exactly the \citet{duan2021pac} network architecture);
a softmax discriminator with a scaling parameter of $100$, i.e., $\mathrm{softmax}(\u) = \frac{e^{100u_i}}{\sum_i e^{100u_i}}$, that takes as input the expected payoffs of each player at the given equilibrium actions predicted by the generator and outputs its softmax;
a less precise softmax discriminator with a scaling parameter of $10$;
and,  a neural network with one linear layer with 1024 nodes and a softmax activation layer with scaling 1 (the total number of parameters for this discriminator is 7,115).  


\paragraph{Training and Hyperparameters.}

We run our algorithm with no inner loop iterations and 10,000 outer loop iterations for the non-neural network discriminators, since they require no training. We adopt for the gradient step in our algorithm 
the ADAM algorithm. We use a learning rate of 0.001 for the optimizer step on each of 
the generator and discriminator  (when appropriate), and use the default settings for the other hyperparameters of ADAM as given in the OPTAX implementation. We process the training data in batches of size 50. 

\paragraph{Experimental Results.} 

In \Cref{fig:gamut_train} (train) and \Cref{fig:gamut_test} (test), we observe that as the quality of the discriminator becomes more approximate the quality of the generator degrades significantly in certain games, underscoring the importance of designing optimal discriminators for \nees{} in certain settings.
Perhaps more interestingly, we observe that  \nees{} with a linear layer discriminator has a hard time in the Bertrand oligopoly and Traveller's Dillemma games. The reason for this is that the discriminator has a hard time learning a pure strategy best-response action, and this seems  crucial for our training algorithm to find an optimal generator in these two games.
This is further justified by \nees{}'s near perfect performance when coupled with 
the true best-response discriminator. In contrast, for other games the neural network's performance suggests that an approximate best-response is enough for our training algorithm to find the optimal discriminator. Future work can investigate the relationship between game classes, and the precision-level w.r.t.~the discriminator that is required for our training algorithms to perform well. We note that \mydef{normalized exploitability} is given as the exploitability divided by the average exploitability over the action space.
% 
\begin{figure*}[t]
  \centering
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\linewidth,trim={0 0 8.5cm 1cm},clip]{figures/gamut/hardmax/facet_train.png}
    \caption{\nees{} with discriminator that outputs the true best-response ($\argmax$ of the expected payoffs for each player).}
  \end{subfigure}
  \hspace{0.5cm}
  \begin{subfigure}{\textwidth}     
    \includegraphics[width=\linewidth,trim={0 0 6.2cm 1cm},clip]{figures/gamut/softmax 100/facet_train.png}
    \caption{\nees{} with discriminator that outputs the softmax of the expected payoffs for each player (scaling parameter 100).}
  \end{subfigure}
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\linewidth,trim={0 0 8.8cm 1cm},clip]{figures/gamut/softmax10/facet_train.png}
    \caption{\nees{} with discriminator that outputs the softmax of the expected payoffs for each player (scaling parameter 10).}
  \end{subfigure}
%   \hspace{0.5cm}

%   \begin{subfigure}{0.3\textwidth}
%     \includegraphics[width=\linewidth]{figures/Arrow-Debreu/CES_GC_exploit_CI1.png}
%     \caption{Caption for image 4}
%   \end{subfigure}
%   \hspace{0.5cm}
%   \begin{subfigure}{0.3\textwidth}
%     \includegraphics[width=\linewidth]{figures/Arrow-Debreu/CES_GS_exploit_CI1.png}
%     \caption{Caption for image 5}
%   \end{subfigure}
%   \hspace{0.5cm}
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\linewidth,trim={0 0 11.2cm 1cm},clip]{figures/gamut/linear/facet_train.png}
    \caption{\nees{} with a neural network discriminator.}
  \end{subfigure}
  \caption{Training Exploitability of \nees{} on five classes of GAMUT games. We observe that the performance of \nees{} degrades significantly in Bertrand oligopoly and traveller's dilemma when the discriminator is not precise enough.\label{fig:gamut_train}}
  %. For Leontief, exploitability descent is not shown, as it performed much worse than either methods. }
\end{figure*}

\begin{figure*}[!ht]
  \centering
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\linewidth,trim={0 0 8.5cm 1cm},clip]{figures/gamut/hardmax/facet_test.png}
    \caption{\nees{} with discriminator that outputs the true best-response ($\argmax$ of the expected payoffs for each player).}
  \end{subfigure}
  \hspace{0.5cm}
  \begin{subfigure}{\textwidth}     
\includegraphics[width=\linewidth,trim={0 0 6cm 1cm},clip]{figures/gamut/softmax 100/facet_test.png}
    \caption{\nees{} with discriminator that outputs the softmax of the expected payoffs for each player (scaling parameter 100).}
  \end{subfigure}
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\linewidth,trim={0 0 8.6cm 1cm},clip]{figures/gamut/softmax10/facet_test.png}
    \caption{\nees{} with discriminator that outputs the softmax of the expected payoffs for each player (scaling parameter 10).}
  \end{subfigure}
%   \hspace{0.5cm}

%   \begin{subfigure}{0.3\textwidth}
%     \includegraphics[width=\linewidth]{figures/Arrow-Debreu/CES_GC_exploit_CI1.png}
%     \caption{Caption for image 4}
%   \end{subfigure}
%   \hspace{0.5cm}
%   \begin{subfigure}{0.3\textwidth}
%     \includegraphics[width=\linewidth]{figures/Arrow-Debreu/CES_GS_exploit_CI1.png}
%     \caption{Caption for image 5}
%   \end{subfigure}
%   \hspace{0.5cm}
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\linewidth,trim={0 0 11cm 1cm},clip]{figures/gamut/linear/facet_test.png}
    \caption{\nees{} with a neural network discriminator.}
  \end{subfigure}
  \caption{Testing Exploitability of \nees{} on five classes of GAMUT games. We observe that the performance of \nees{} degrades significantly in Bertrand oligopoly and traveller's dilemma
  when the discriminator is not precise enough.\label{fig:gamut_test}}
  %. For Leontief, exploitability descent is not shown, as it performed much worse than either methods. }
\end{figure*}




==> Learning Generalized Nash Equilibrium - ICML/generalization.tex <==

\subsection{Generalization bounds.}
We also give a sample complexity result for the  
empirical exploitability, showing how cumulative regret can be approximated 
with a sample of pseudo-games that is polynomial in the parameters of the game distribution, 
$\nicefrac{1}{\varepsilon}$ and $\nicefrac{1}{\delta}$.
%, the desired precision levels for the approximation.
%
The novelty of the result comes from  the  context: 
we mentioned earlier that expected exploitability need not be 
Lipschitz-continuous, making it hard 
to use any standard and simple machinery to prove a  sample complexity
bound.   However, by reframing this problem 
as one of learning the expected cumulative regret, which is  Lipschitz-continuous, we can obtain the result.
%
%The proof makes use of  standard tools such as covering numbers. to obtain sample complexity bounds. 
%
%
% , which by \Cref{assum:main} is guaranteed to be Lipschitz-smooth. We show in the next theorem that when the expected cumulative regret is sample-efficiently learnable.
%
\begin{restatable}[Sample Complexity of Expected Cumulative Regret]{theorem}{thmsamplecomplexity}\label{thm:sample_complexity}
For any hypothesis classes $\hypotheses \subset \actions[][\pgames]$, $\otherhypotheses \subset \actionspace^{\actions \times \pgames}$ $\varepsilon, \delta \in (0,1)$ and any pseudo-game distribution $\distribpgames \in \simplex(\pgames)$, with probability at least $1-\delta$ over draw of the training set $\samplepgames \sim \distribpgames^\numsamples$ with 
    $\numsamples \geq \frac{9 }{\varepsilon^2} \left[ \log\left(\frac{\coveringcard(\hypotheses, \nicefrac{\varepsilon}{6})}{\delta}\right) + \log\left(\frac{\coveringcard(\otherhypotheses, \nicefrac{\varepsilon}{6})}{\delta}\right) \right]$,
we have:
\begin{align*}
    \left| \mathop{\Ex}_{\pgame \sim \mathrm{unif}(\samplepgames)} \! \left[\cumulregret[][\pgame](\hypothesis(\pgame), \otherhypothesis(\pgame, \hypothesis(\pgame))) \right] \!\!- \!\! \mathop{\Ex}_{\pgame \sim \distribpgames} \! \left[\cumulregret[][\pgame](\hypothesis(\pgame), \otherhypothesis(\pgame, \hypothesis(\pgame))) \right] \right| \leq \varepsilon
\end{align*}
\end{restatable}



% $\left\{\batchpgames[1], \hdots, \batchpgames[\numbatches] \right\} \subset \samplepgames$. 


% when formulated this way making it of little practical relevance for learning parametric function approximators, e.g., deep neural networks, since it is not possible to compute and (sub)gradients of the function and optimize the some parameter of the exploitability using a first order method. We make the following observation which allows us to first order methods to optimize the exploitability:


% \vspace{-5mm}
% \begin{align*}
% \exploit[][\pgame](\action) 
% = \sum_{\player \in \players}  \max_{\otheraction[\player] \in \actions[\player](\naction[\player])} \regret[\player][\pgame](\action[\player], \otheraction[\player]; \naction[\player]) %\label{eq:sum_max}
% = \max_{\otheraction \in \actions(\action)}  \sum_{\player \in \players} \regret[\player][\pgame](\action[\player], \otheraction[\player]; \naction[\player]) %\label{eq:max_sum}
% = \max_{\otheraction \in \actions(\action)}  \cumulregret(\action, \otheraction)
% \end{align*}


% This lemma tells us that we can reformulate GNEP as the quasi-optimization problem of minimizing exploitability, i.e., $\min_{\action \in \actions(\action)} \exploit[][\pgame](\action)$, or min-maxing cumulative regret, i.e., $\min_{\action \in \actions(\action)} \max_{\otheraction \in \actions(\action)}  \cumulregret(\action, \otheraction)$.
% Here, ``quasi'' refers to the fact that a solution to this problem is both a minimizer of $\exploit[][\pgame]$ \emph{and\/} a fixed point $\action^*$ s.t.\ $\action^* \in \actions(\action^*)$. 


% \paragraph{Digression} Although the fixed point aspect of this problem makes it hard to compute a GNE, since the order of the minimum operations can be exchanged, we can decompose the outer minimization problem into $\numplayers$ minimization problems:
% \begin{align}
%     \min_{\action[1] \in \actionspace[1]} \min_{\action[2] \in \cup_{\naction[2] \in \actionspace[-1,-2]}\actions[2](\action[1], \naction[2])}
%     \hdots
%     \min_{\action[\numplayers] \in \actions[\numplayers](\naction[\numplayers])}
%     \max_{\otheraction \in \actions(\action)}  \cumulregret(\action, \otheraction)
% \end{align}


% The advantage of this reformulation is that it does away with the problem of simultaneously minimizing a function and solving for a fixed point problem, a problem for which no algorithms are known, and turns it into a sequential optimization problem. Even though such problems are in general NP-hard \cite{dempe2002foundations}, a local solution to such problems can often be found. This is quite desirable since very little is known on solving pseudo-games which are not jointly convex. More precisely, using the envelope theorem \cite{afriat1971envelope, milgrom2002envelope}, one can differentiate through each optimization problem to run a sequential gradient method which one would hope would converge to a stationary point of the exploitability. We note that although this approach seems very similar to that of backpropagation to obtain a direction of descent for neural network parameters, it is an inherently different method since backpropagation would make use of the implicit function theorem and the chain rule, while this approach calls for the computationally more appealing envelope theorem.


% \paragraph{Jointly Convex Pseudo-Games} When the pseudo-game is additionally assumed to have joint constraints, then the VEs of the pseudo-game can be solved as an exploitability minimiza tion problem and can be expressed as an even nicer min-max optimization problem:
% \begin{align}
%     \min_{\action \in \actions} \max_{\otheraction \in \actions}  \cumulregret(\action, \otheraction)
% \end{align}

% We focus on this simpler problem for the moment and propose the following algorithm to minimize exploitability:




==> Learning Generalized Nash Equilibrium - ICML/intro.tex <==
\section{Introduction}

Economic models and  equilibrium concepts %dcp (e.g., \cite{walras, arrow-debreu})
are critical tools to solve practical problems, including capacity allocation in wireless and network communication \cite{han2011wireless, pang2008distributed}, energy resource allocation~\cite{hobbs2007power, wei1999power}, and cloud computing~\cite{gutman2012fair, lai2005tycoon, zahedi2018amdahl, ardagna2017cloud}. 
% Although, the computation of equilibrium in these models is intractable in the worst-case, in practice, many applications only require an approximate solution in expectation over a distribution of problem instances.
% 
% Equilibrium-based modelling, arguably first introduced into economics in the works of \citeauthor{cournot1897researches} \cite{cournot1897researches} and \citeauthor{walras} \cite{walras}, has nowadays become one of the main paradigms in mathematical economics 
% % (see for instance this year's Nobel laureates in economics \cite{diamond1983bank})
% with the seminal works of \citeauthor{arrow-debreu} \cite{arrow-debreu} and \citeauthor{mckenzie1954equilibrium} \cite{mckenzie1954equilibrium} establishing the existence of equilibrium prices in a very broad model of an economy.
%dcp Although some of these economic models can be cast as games \cite{nash1950existence}, i.e., models of rational interaction, many  
%
Many of these economic models %(e.g., \cite{arrow-debreu}) are instances of a more general model of rational interaction known as
are instances of what are known as \mydef{pseudo-games}, in which the actions taken by each player affect not only the other players' payoffs, as in games, but also the other players' strategy sets.\footnote{In many games, such as chess, the action taken by one player affects the actions available to the others, but these games are sequential, while in pseudo-games actions are chosen simultaneously. % 
Additionally, even if one constructs a game with payoffs that penalize the players for actions that are not allowed, the NE of the ensuing game will in general not correspond to the GNE of the original pseudo-game and can often be trivial. We refer the reader to \Cref{sec_app:gne_vs_ne} for a mathematical example.} 
%
The formalism of pseudo-games was introduced by \citet{arrow-debreu}, who used
it in studying their foundational microeconomic equilibrium model, the competitive economy model.
%of competitive economy is a pseudo-game \cite{arrow-debreu}.

% \mydef{Games} consist of a set of players, each of whom simultaneously chose an action from an action space, and receive a payoff based on all the players actions. A \mydef{Nash equilibrium} (NE)  \cite{cournot1897researches,nash1950existence} is a \mydef{policy profile}, i.e., a collection of actions for all players, one per player, for which no player can improve their payoff by unilaterally deviating to another action in their action space. \mydef{Pseudo-games} are a \emph{generalization} of games, in which the \emph{simultaneous} actions taken by each player affect not only the other players' payoffs, as in games, but also the other players' action spaces.

%
The standard solution concept for pseudo-games is the {\em generalized Nash equilibrium (GNE)} \cite{arrow-debreu, facchinei2010generalized}, which is an action profile from which no player can improve their payoff by unilaterally deviating to another action in the space of admissible actions determined by the actions of other players. Important economic models can often be formulated as a pseudo-game, with their set of solutions equal to the set of GNE of the pseudo-game: for instance, the set of {
\em competitive equilibria (CE)}~\cite{walras,arrow-debreu} of an Arrow-Debreu competitive economy corresponds to the set of GNE of an 
associated pseudo-game.
%

A large literature has been devoted to the computation of GNE in certain classes of pseudo-games but unfortunately many algorithms that are guaranteed to converge in theory have in practice been observed to converge slowly in ill-conditioned or large problems or fail numerically~\cite{facchinei2010penalty, jordan2022gne, goktas2022exploitability}. Additionally, all known algorithms have hyperparameters that have to be optimized individually for every pseudo-game instance \cite{facchinei2010generalized}, deteriorating the performance of these algorithms when used to solve multiple pseudo-games. These issues point to a need to develop methods to compute GNE, for a distribution of pseudo-games, reliably and quickly.
% Another more concrete problem that can be modeled as a pseudo-game (but not  as a game) is that of
% power allocation over wired telecommunication networks
% %under the Gaussian
% %frequency-selective interference channel model 
% \cite{pang2008distributed}.  Here, each  wire in a cable can be modeled as a player who is picking a power allocation, 
% with the goal of minimizing total power consumption while achieving a minimum transmission rate. As a result of interference, the  transmission rate of a wire depends on the power allocated to each  wire in the cable, which
% means that the  choice of power for a wire  to meet the minimum transmission rate 
% depends on the power allocations of others, making this  a pseudo-game.

% \if 0
% Information on telecommunication networks is carried via signals sent through wires. Due to the electromagnetic coupling within and across wires, more power sent through a bundle of wires, i.e., a cable, can lead to a degradation of quality of service. That is, the transmission quality for a wire is a function of the power allocated to the wires within a cable. At a high level, the problem of network carriers is to achieve a minimum desired transmission rate through each wire, while minimizing total power consumption across all wires. This problem is an economic problem, in particular, one of resource allocation, and hence can be modelled as a pseudo-game in which each player is a wire, and the goal of the players is to minimize the total power consumption while guaranteeing a minimum transmission rate through each wire. We note that this problem cannot be modelled as a game, due to the constraint that the transmission rate of a wire, which is dependent on the power allocated to all wires within the same cable, has to be above a certain threshold.\footnote{Even if one constructs a game with payoffs that penalize the players for actions that are not allowed, the NE of the ensuing game will in general not correspond to the GNE of the original pseudo-game and can often be trivial. We refer the reader to \Cref{sec_app:gne_vs_ne} for a mathematical example.}
% \fi


% Our approach amortizes computational cost up-front at training time, and allows for near constant-cost evaluation time at inference time, and comes with theoretical guarantees on its computational and sample complexity \Cref{sec:theory}, making it a good fit to various applied contexts which we demonstrate with experiments on normal-form games (\Cref{sec_app:experiments}), Arrow-Debreu competitive economies, and a model of the Kyoto joint implementation mechanism (\Cref{sec:experiments}).

We reformulate the problem of computing GNE in pseudo-games (and CE in Arrow-Debreu competitive economies) as a learning problem for a generative adversarial network (GAN) called the \mydef{Generative Adversarial Equilibrium Solver (\nees{})},
consisting of a generator and a discriminator network. 
The generator takes as input a parametric representation of a pseudo-game, and predicts a solution that
consists of a tuple of actions, one per player.
The discriminator takes as input both the pseudo-game and the output of the generator, and outputs a best-response for each player,
seeking to find a useful unilateral deviation for all players; this also gives  the sum of regrets,
with which to evaluate the generator (see \Cref{fig:network_diagram}). \nees{} predicts GNE and CE in batches and in order to minimize the expected exploitability, across a distribution of pseudo-games. \nees{} amortizes computational cost up-front in training, and allows for near constant evaluation time for inference. Our approach is inspired by previous methods that cast the computation of an equilibrium in normal-form games as an unsupervised learning problem~\cite{duan2021pac,marris2022cce}.
These methods train
a network to predict a strategy profile that minimizes  the \mydef{exploitability}  (i.e., the sum of the players' payoff-maximizing unilateral deviations w.r.t.\ a given strategy profile)
over a distribution of games. These methods become inefficient in pseudo-games, since in contrast to regular games, the exploitability in pseudo-games (1) requires solving a non-linear optimization problem, (2) is not Lipschitz-continuous, in turn making it hard to learn from samples, and (3) has unbounded gradients, which might lead to exploding gradients in neighborhoods of GNE. Our GAN formulation  circumvents all three of these issues.

Although the computation of GNE is intractable in the worst-case \cite{chen2006settling, daskalakis2009complexity, chen2009spending, vazirani2011market, garg2017settling}, in practice,  applications may only require a solver that gives solutions with high accuracy in
expectation over a realistic distribution of problem instances. 
In particular, a decision maker may need  to compute a GNE for a sequence of  pseudo-games from some family 
%
or \emph{en masse} over a 
set of pseudo-games 
sampled from some distribution of interest. 
%
%
An example of such an application is the problem of resource allocation on cloud computing platforms \cite{hindman2011mesos,isard2009quincy, burns2016borg,vavilapalli2013apache} where a significant number of methods make use of repeated computation of competitive equilibrium \cite{gutman2012fair, lai2005tycoon, budish2011combinatorial, zahedi2018amdahl, varian1973equity} and generalized Nash equilibrium \cite{ardagna2017cloud, ardagna2011cloud, ardagna2011flexible, anselmi2014generalized}. In such settings, as consumers request resources from the platform, the platforms have to find a new equilibrium  while handling all numerical failures within a given time frame.
% Going back to the telecommunication example, a national network carrier has to make a
% rapid decision of how to send power through cables,  as it receives a communication request, and it has to do this {\em en masse}, not just for one cable infrastructure in one town, but for the cable infrastructures across multiple towns, 
% requiring them solve a batch of pseudo-games. 
Another example is policy makers who often want to understand the equilibria induced by a policy for different distributions of agent preferences in a pseudo-game %
allowing them to study the impact of a policy for a distribution on different possible kinds of participants. For example,
in studying the impact of a protocol such
as the \mydef{Kyoto joint implementation mechanism} (see \Cref{sec:experiments}), one might be interested in understanding how the emission levels of countries would change based on their productivity levels \cite{roger2000kyoto}.
%,
%in which case they are interested in solving many different
%pseudo-games \cite{breton2006game}; 
%we show that our method can handle such applications by replicating existing theoretical analysis of the Kyoto joint implementation mechanism in \Cref{sec:experiments}.
%
%
Other applications 
%with the same requirement include state-value function-based reinforcement leaning algorithms for solving
include computing competitive equilibria
%, an example of GNE,
in stochastic market environments. 
For example,  %algorithms such as Model-based Optimistic Online Learning for Markov Exchange Economy and  Model-based Pessimistic Online Learning for Markov Exchange Economy
%iteratively construct better state value functions which determine a new 
recently proposed algorithms
work through a series of equilibrium problems, each of which has to be solved quickly~\cite{liu2022welfare}.
%dcp or similar online learning algorithms such as randomized exchange equilibrium learning \cite{guo2022onlineEE} which compute a competitive equilibrium when agents' payoffs can only be obtained from sample observations also require solving for a competitive equilibrium iteratively and quickly. 
% \input{figures/figure_intro_model}
%Critically, these applications require one to approximately compute a CE or a GNE in a quick fashion while handling any numerical failures that might occur in practice with different input types. 
%even where there exists no known algorithms to compute such solutions. 
%

% \nees{} is a {\em generative adversarial network} (GAN) that learns to 
% map pseudo-games to  GNE. 
% Similar to previous approaches, the \nees{} method predicts equilibria so as to minimize distance from equilibrium in payoff space, over a distribution of pseudo-games. 
% 
\input{contributions}
% 
\input{figures/figure_intro_network}
% 
\input{related}

==> Learning Generalized Nash Equilibrium - ICML/kyoto.tex <==
\subsection{Kyoto Joint Implementation Mechanism}

\paragraph{Experimental Setup}
For this experiment, we focus on computing a refinement of the GNE known as VE (see \Cref{sec_ap:prelims}),
which are guaranteed to exist for this jointly convex pseudo-games.\footnote{We recall that a mydef{variational equilibrium (VE)} (or \mydef{normalized GNE}) of a pseudo-game is a strategy profile $\action^* \in \actions$ s.t.\ for all $\player \in \players$ and $\action \in \actions$, $\util[\player](\action^*) \geq  \util[\player](\action[\player], \naction[\player][][][*])$. See \Cref{sec_ap:prelims} for more details.} %
This does not change the structure of the generator of \nees{} or the training algorithm.
However, it allows us to consider discriminators that output best-responses that are in the space of jointly feasible actions rather than in the space of individually feasible action spaces, greatly simplifying the architecture of our discriminator.  We aim to first replicate the results provided in section 4 of \citeauthor{breton2006game} \cite{breton2006game}. To do so, we first consider a 2 country Kyoto JI mechanism, with all parameters of the Kyoto JI mechanism except $\revrate$ fixed, and compute equilibria for different values of $\revrate$ (\Cref{fig:phase_kyoto}). We then also consider a 2 country Kyoto JI mechanism where we sample all parameters randomly (\Cref{fig:exploit_kyoto}).

\paragraph{Pseudo-Game Generation.}
We sample 12,000 pseudo-games, putting
aside 1,000 for validation and 1,000 for testing. 
We sample the payoff and constraint parameters  of all the players ($\revrate$, $\investrate$, $\emitcap$, $\damagerate$), uniformly in the range $[0.5, 50]$ to produce the pseudo-games.
%
For each of these pseudo-games, since the set of jointly feasible actions is a polytope, we also generate the vertices associated with the set of jointly feasible actions. To do so, we use the pycdd library \cite{pycddlib2015}, and store a matrix of vertices for each pseudo-game, where the rows correspond to the maximum number of vertices, denoted $\mathrm{MaxNumVertex}$, for any pseudo-game in the training set, and the columns correspond to the dimension of the action space, i.e., $\numcountries*(\numcountries + 1)$ (the first row corresponds to emissions, the  last $\numcountries$ rows correspond to the investment matrix).
For the experiments, and replicating the comparative static analysis of \citet{breton2006game}, 
we randomly sample and fix all parameters of the game except $\revrate$, and
sample $\revrate$ from the range $[0.5, 50]^\numcountries$ as stated above. 

\paragraph{Hyperparameters.}
%
We run our algorithm with an initial warm-up of 10,000 iterations for the discriminator. This warm-up procedure follows exactly the inner loop of \Cref{alg:cumul_regret} but instead uses randomly sampled pseudo-games and randomly sampled action profiles. After the warmup, we use only one step of inner loop iteration for running \Cref{alg:cumul_regret} and run the outer loop for 10,000 iterations. Together with the warmup, the small number of inner loop iterations allow us to significantly speed up the training process. The gradient step in our algorithm is a step of the ADAM algorithm. For the discriminator, we use the same learning rate for the warm-up and regular training, following a grid search which is a learning rate of $0.0001$, while for the generator we use a learning rate of $0.001$. 

\paragraph{Generator Architecture.}
%

\begin{figure}[!ht]
    \centering
    \includegraphics[width=\linewidth]{architectures/Kyoto_gen.png}
    \caption{Architecture of the generator of \nees{} for Kyoto JI mechanisms.}
    \label{fig:kyoto_gen}
\end{figure}

We summarize the architecture of \nees{}'s generator for Kyoto JI mechanisms in \Cref{fig:kyoto_gen}. The generator for the Kyoto setting
takes as input the game matrix ($\revrate$, $\investrate$, $\emitcap$, $\damagerate$),
and feeds these inputs through a neural network with two hidden layers, each
with 20 and 30 nodes respectively and ReLU activations.
%
The output of each layer is also passed through a ReLU
activation, as well as a BatchNorm \cite{ioffe2015batch} layer with trainable parameters, 
and with default parameters as implemented by Haiku.
The output layer of the neural network consists of a fully connected layer with softmax activation with output dimension equal to $\mathrm{MaxNumVertex}$. The output of this final layer is  multiplied with the matrix of vertices associated with the pseudo-game ($\revrate$, $\investrate$, $\emitcap$, $\damagerate$) across its rows, i.e., each vertex associated with pseudo-game's constraint is multiplied by some probability.
The obtained matrix is then summed up across the rows and output by the generator after setting the first column to be $\emit$, and the matrix formed by the remaining columns to be $\invest$. Since the neural network outputs a convex combination of the vertices associated with the constraints of the game, the action profile outputted by the neural network is always jointly feasible. The number of parameters for the generator is 2,824.


\paragraph{Discriminator Architecture}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=\linewidth]{architectures/Kyoto_discrim.png}
    \caption{Architecture of the generator of \nees{} for Kyoto JI mechanisms.}
    \label{fig:kyoto_discrim}
\end{figure}

We summarize the architecture of  \nees{}'s discriminator for Kyoto JI mechanisms in \Cref{fig:kyoto_discrim}.Our discriminator takes as input the matrix $(\emit, \invest)$, the output of the generator,
and the pseudo-game matrix ($\revrate$, $\investrate$, $\emitcap$, $\damagerate$).
The equilibrium $(\emit, \invest)$ is first passed through a neural network with two fully connected 
trainable BatchNorm layers, each with 500 nodes.
%
Similarly, the pseudo-game ($\revrate$, $\investrate$, $\emitcap$, $\damagerate$) is passed through a network with the same architecture. The output of both networks are then concatenated over the last dimension, i.e., the matrices outputted by both networks are appended horizontally so as to preserve the number of rows $\numcountries$.
and passed through a neural network with two fully connected trainable BatchNorm layers, each
with 500 nodes.
For each of these layers, the output  is passed through a ReLU
activation. The output of the last neural network is then flattened and passed through a final fully connected layer with a softmax activation. The output of this final layer is  multiplied with the matrix ($\revrate$, $\investrate$, $\emitcap$, $\damagerate$) of vertices associated with the pseudo-game across its rows.
%
The obtained matrix is then summed up across the rows and output by the discriminator after setting the first column to be $\emit$, and with the matrix formed by the remaining columns of the output adopted as 
$\invest$. Since the neural network outputs a convex combination of the vertices associated with the constraints of the game, the action profile is always jointly feasible, meaning that the neural network outputs a best-response (for a VE). The number of parameters for the discriminator is 1,302,544.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/kyoto/kyoto_phase_exploit.png}
    \caption{Normalized exploitability achieved by \nees{} throughout training for a two country JI mechanism.
    \label{fig:exploit_kyoto}}
\end{figure}

==> Learning Generalized Nash Equilibrium - ICML/learning.tex <==
\section{Generative Adversarial Learning of Equilibrium Mappings}\label{sec:GAN}

% 
In this section, we revisit previous formulations of the problem of learning an equilibrium mapping, discuss the computational difficulties associated with these formulations when used to learn GNE, and introduce our generative adversarial learning formulation. 

% A first approach to learn an equilibrium mapping is to consider the problem as a supervised 
% learning problem, where one has access to a joint distribution of (pseudo-game, GNEs) pairs, and learns a mapping that minimizes  error over this distribution. 
% This approach does not scale in the present setting, 
% because it requires us to generate GNE for a diverse enough sample of pseudo-games (another difficulty is that it requires an approach for equilibrium selection).
% \if 0 
% More precisely, for any pseudo-game $\pgame \in \pgames$, let $\actionspace^*(\pgame)$ be the set of GNE of $\pgame$. Consider a 
% \mydef{hypothesis class} $\hypotheses \subseteq \actions[][\pgames]$, i.e., a subset of all mappings from games to jointly feasible actions, and a distribution over pseudo-games $\distribpgames \in \simplex(\pgames)$, the \mydef{supervised learning problem} consists of finding an \mydef{hypothesis} $\hypothesis^*\in \hypotheses$ such that $\hypothesis^* \in \argmin_{\hypothesis \in \hypotheses} \Ex_{\pgame \sim \pgames} \left[\mathbbm{1}_{\hypothesis(\pgame) \notin \actionspace^*(\pgame)} \right]$. Unfortunately, this supervised learning approach is computationally intractable \cite{marris2022cce, zhijian2021ne}, since 1) the error function requires us to generate all GNE of the pseudo-game $\pgame$, $\Ex_{\pgame \sim \pgames} \left[\mathbbm{1}_{\hypothesis(\pgame) \notin \action^*(\pgame)} \right]$ ill-defined without adequate equilibrium selection, and 2) requires us to generate GNE for a diverse enough sample of pseudo-games, i.e., beyond tractable cases, both of which are hard since GNEP is in general intractable. Note that the former issue cannot be remedied by comparing the distance of the payoff profiles associated with the strategy profile predicted by the equilibrium mapping and that of an arbitrary GNE, because the equilibrium payoffs of GNE differ from one another unless the pseudo-game is zero-sum.
% \fi
%

%
% .
As creating a sufficiently diverse sample of (pseudo-game, GNE) pairs, while performing adequate equilibrium selection, is intractable both theoretically and computationally, we forgo of supervised learning methods, and formulate the equilibrium mapping learning problem as an \mydef{unsupervised} learning problem, 
following the approach adopted by~\citet{marris2022cce,zhijian2021ne} for finding Nash equilibria.
%
Given a hypothesis class $\hypotheses \subseteq \actions[][\pgames]$, and a distribution over pseudo-games $\distribpgames \in \simplex(\pgames)$, \mydef{the unsupervised learning problem} for an equilibrium mapping consists of finding a hypothesis $\hypothesis^* \in \argmin_{\hypothesis \in \hypotheses} \Ex_{\pgame \sim \distribpgames} \left[\ell(\pgame, \hypothesis(\pgame))\right]$ where  $\ell: \pgames \times \actionspace \to \R$ is a loss function that outputs the distance of $\action \in \actionspace$ from a GNE,
such that for any pseudo-game $\pgame \in \pgames$, $\ell(\pgame, \action^*) = 0$ iff $\action^*$ is a GNE of $\pgame$.
In particular, \citet{marris2022cce, zhijian2021ne} suggest to use   exploitability
as the loss function.
%, i.e., $\ell(\pgame, \cdot) = \exploit[][\pgame](\cdot)$.
% \if 0
% % Note that in general, unless $\hypotheses = \actions[][\pgames]$, we are not guaranteed the existence of an equilibrium mapping $\hypothesis \in \hypotheses$ such that $\Ex_{\pgame \sim \distribpgames} \left[\exploit[][\pgame](\hypothesis(\pgame)) \right] = 0$. That is, is in general, unless $\hypotheses = \actionspace^\pgames$ the problem is unrealizable.\footnote{Note that by Arrow-Debreu's lemma on abstract economies, the problem is guaranteed to be realizable for $\hypotheses = \actions[][\pgames]$.}
% % Unfortunately, the exploitability in pseudo-games is non-differentiable and non-convex. Perhaps even more incovenvenient is that even when the payoffs $\util$, and constraints $\actionconstr$ are Lipschitz-continuous, the exploitability in pseudo-games is not in general Lipschitz-continuous (see \Cref{ex:non_lipschitz_exploitability}). This is in stark contrast with the exploitability when the pseudo-game is a game, where it is guaranteed to be Lipschitz-continuous. The reason for why the Lipschitz-continuity of the exploitability in games does not generalize to pseudo-games, is that the inputs of the exploitability $\action$ parameterize the constraints in the optimization problem defining each player's maximal regret computation, i.e., $\max_{\otheraction[\player] \in \actions[\player](\naction[\player])} \regret[\player][\pgame](\action[\player], \otheraction[\player]; \naction[\player])$, and optimal values of optimization problems are not Lipschitz continuous in their parameters when the parameters determine the constraints \cite{}! 
% \fi
However, a number of  issues  arise when trying to minimize the expected exploitability over a distribution of pseudo-games:

(1) Computing the gradient of the exploitability, when it exists, for even only one pseudo-game requires solving a concave maximization problem
%, making the computation of the gradient of the expected exploitability costly as it requires to solve as multiple concave optimization problems. We note that 
(this reasoning also applies to continuous games).

(2) The exploitability in pseudo-games, is in general not Lipschitz-continuous (unlike in regular games), even when payoffs are Lipschitz-continuous, since the inputs of the exploitability parameterize the constraints in the optimization problem defining each player's maximal regret computation.
%
This makes it unclear how
to efficiently approximate $\Ex_{\pgame \sim \distribpgames} \left[\exploit[][\pgame](\action) \right]$ from samples, without knowledge of the distribution.
% \if 0
% efficiently obtain estimates of the expected exploitability, $\Ex_{\pgame \sim \distribpgames} \left[\exploit[][\pgame](\action) \right]$,
% from a sample of pseudo-games $\distribpgames$.


% This is unfortunate as it suggests that
% % because if one wants to approximate $\Ex_{\pgame \sim \distribpgames} \left[\exploit[][\pgame](\action) \right]$ from samples without knowledge of the distribution, as one does often in practice \cite{} since computing the expected exploitability in closed form is intractable in general, without Lipschitz-continuity of $\exploit[][\pgame](\action)$, $\Ex_{\pgame \sim \distribpgames} \left[\exploit[][\pgame](\action) \right]$ is also not guaranteed to be Lipschitz-continuous, and as a result 
% one cannot approximate $\Ex_{\pgame \sim \distribpgames} \left[\exploit[][\pgame](\action) \right]$ with an efficient sample size, i.e., a sample size polynomial in the parameters of the pseudo-game, as it is often the case \cite{kearns1994introduction}
% \fi
%

(3) The exploitability in pseudo-games  is absolutely continuous and hence differentiable almost everywhere \cite{afriat1971envelope}, but in contrast to games, the gradients   cannot be bounded. This in turn precludes the convergence of first-order methods.\footnote{
%Note that while exploitability is also not guaranteed to be differentiable in games, it is guaranteed to Lipschitz-continuous. 
We refer the reader to \Cref{sec_app:examples} for an example in which exploitability is not Lipschitz-continuous and has unbounded gradients.}
% \smallskip


% Although finding such a mapping is desirable, unless the problem is realizable, i.e., there exists an equilibrium mapping $\hypothesis^*: \pgames \to \actionspace$ such that for all pseudo-games $\pgame \in \pgames$, $\exploit[][\pgame](\pgame, \hypothesis^*(\pgame)) = 0$



%  . One solution to the learning problem is the robust equilibrium mapping which requires one to 1) construct a loss function  $\exploit[][\pgame]: \pgames \times \actionspace \to \R$ which for each pseudo-game $\pgame \in  \pgames$ and action profile $\action \in \actionspace$ outputs the distance of $\action$ from a GNE such that for any $\pgame \in \pgames$, $\exploit[][\pgame](\pgame, \action^*) = 0$ if $\action^*$ is a GNE of $\pgame$, and 2) using the loss $\exploit[][\pgame]$, to learn a \mydef{robust equilibrium mapping} $\hypothesis^* \in \actionspace^{\pgames}$ such that $\hypothesis^* \in \argmin_{\hypothesis \in \actionspace^\pgames} \max_{\pgame \in \pgames} \exploit[][\pgame](\pgame, \hypothesis(\pgame)) = 0$. Although finding such a mapping is desirable, unless the problem is realizable, i.e., there exists an equilibrium mapping $\hypothesis^*:: \pgames \to \actionspace$ such that for all pseudo-games $\pgame \in \pgames$, $\exploit[][\pgame](\pgame, \hypothesis^*(\pgame)) = 0$, it seems unlikely such a mapping could be easily found since Nash equilibria are highly discontinuous in the parameters of the games \cite{scalzo2019continash} Instead, one might consider minimizing loss over a distribution of games $\distribpgames \in \simplex(\pgames)$, rather than all games and finding an \mydef{approximate equilibrium mapping}  $\hat{\hypothesis} \in  \argmin_{\hypothesis \in \actionspace^\pgames} \mathop{\Ex}_{\pgame \sim \distribpgames} \left[\exploit[][\pgame](\pgame, \hypothesis(\pgame)) \right]$. With our learning problem now formulated we now turn our attention to 1) formulating a loss to learn an approximate equilibrium mapping, and then 2) provide an algorithm to compute such a mapping.

% \begin{restatable}{lemma}{lemmaNoExploitGne}
% \label{lemma:no_exploit_gne}
% Given a pseudo-game $\pgame$, for all $\action \in \actionspace$, $\exploit[][\pgame](\action) \geq 0$ and $\exploit[][\pgame](\action) = \max_{\otheraction \in \actions(\action)} \cumulregret(\action, \otheraction)$.
% Additionally, a strategy profile $\action^* \in \actions(\action^*)$ is a GNE iff it achieves the lowerbound, i.e., $\exploit[][\pgame](\action^*) = 0$.
% \end{restatable}



% \begin{example}\label{ex:non_lipschitz_exploitability}[Continuous Action Space Game]
% Consider a two-player zero-sum pseudo-game with action space $\actionspace[1] = \actionspace[2] = 
% [0, 1]$, payoffs $\util[1](\action[1][ ], \action[2][ ]) = -\util[2](\action[1][ ], \action[2][ ]) = \action[1][ ]\action[2][ ]^{\nicefrac{3}{2}}$, and constraints $\actionconstr[1][ ](\action[1][ ], \action[2][ ]) = 1 - \action[1][ ] (\action[2][ ])$
% % , $\actionconstr[2][ ](\action[1][ ], \action[2][ ]) = \action[2][ ] (\action[1][ ])^2 - 1$
% . The exploitability of this pseudo-game is given by 
% \begin{align}
%     \exploit(\action) &=  \max_{(\otheraction[1][ ], \otheraction[2][ ]) \in [0,1]^2: 1 - \otheraction[1][ ] (\action[2][ ]) \geq 0} \otheraction[1][ ]\action[2][ ]^{\nicefrac{3}{2}} - \action[1][ ]\otheraction[2][ ]^{\nicefrac{3}{2}}\\
%     &= \max_{(\otheraction[1][ ], \otheraction[2][ ]) \in [0,1]^2: \frac{1}{(\action[2][ ])} \geq \otheraction[1][ ]} \otheraction[1][ ]\action[2][ ]^{\nicefrac{3}{2}} - \action[1][ ]\otheraction[2][ ]^{\nicefrac{3}{2}}\\
%     % 
%     &= \left\{ \begin{array}{cc}
%     \sqrt{\action[2][ ]}  & \text{ if $\frac{1}{(\action[2][ ])} 
%     \leq 1$}\\
%     \action[2][ ]^{\nicefrac{3}{2}} & 
%     \text{Otherwise}
%     \end{array}\right.
% \end{align}
% \noindent
% Note that the payoffs $\util$ and constraints $\actionconstr$ are both Lipschitz-continuous, however, whenever $\action[1][ ] = 0$ or $\action[2][ ] = 0$, the exploitability grows unboundedly and hence exploitability is not Lipschitz continuous.  
% \end{example}

To address the aforementioned issues, we propose a generative adversarial learning formulation of the associated 
unsupervised learning problem for equilibrium mappings.
The formulation relies on the following observation, whose proof is deferred to \Cref{sec_app:proofs}: the exploitability can be computed \emph{ex post} after computing the expected cumulative regret by optimizing over the space of best-response functions from pseudo-games to actions, 
rather than the space of actions individually for every pseudo-game.
%
\begin{restatable}{observation}{obsganeq}\label{obs:gan_eq}
For any $\distribpgames \in \simplex(\pgames)$, we have:
\begin{align}
    &\min_{\hypothesis \in \actions[][\pgames]} \Ex_{\pgame \sim \distribpgames} \left[\exploit[][\pgame](\hypothesis(\pgame)) \right]  \notag \\
    &= \min_{\hypothesis \in \actions[][\pgames]} \max_{\substack{\otherhypothesis \in \actionspace^{\pgames}: \forall \pgame \in \pgames,\\ \otherhypothesis(\pgame) \in \actions[][\pgame](\hypothesis(\pgame))}}  \Ex_{\pgame \sim \distribpgames} \left[ \cumulregret[][\pgame](\hypothesis(\pgame), \otherhypothesis(\pgame))\right].\label{eq:gan_obs}
\end{align}
\end{restatable}
% 
\noindent
By Arrow-Debreu's lemma on abstract economies~\cite{arrow-debreu}, $\hypothesis^*$ is guaranteed to exist and is an equilibrium mapping iff  $\hypothesis^* \in  \argmin\limits_{\hypothesis \in \actions[][\pgames]} \max\limits_{\substack{\otherhypothesis \in \actionspace^{\pgames \times \actions}: \forall \pgame \in \pgames, \\ \otherhypothesis(\pgame, \hypothesis(\pgame)) \in \actions[][\pgame](\hypothesis(\pgame))}}  \Ex_{\pgame \sim \distribpgames} \left[ \cumulregret[][\pgame](\hypothesis(\pgame), \otherhypothesis(\pgame))\right]$.

This  problem formulation allows us to overcome issues (1) and (2).  For (1), rather than solve 
a concave program to compute the exploitability for each pseudo-game and action profile, 
we can learn a function that maps action profiles to their associated best-response profiles (see for example~\citet{lanctot2017unified} for training best-response oracles).
For (2),  the objective function in \Cref{eq:gan_obs} is Lipschitz-continuous when payoff functions are,  which  opens the doors to use standard proof techniques to learn the objective from a polynomial sample of pseudo-games. 

Still, the gradient of $\max_{\otherhypothesis}\Ex_{\pgame \sim \distribpgames} \left[ \cumulregret[][\pgame](\hypothesis(\pgame), \otherhypothesis(\pgame; \hypothesis(\pgame)))\right]$ with respect to $\hypothesis$ is  in general unbounded even when it exists,
due to the constraint $\forall \pgame \in \pgames, \otherhypothesis(\pgame) \in \actions(\hypothesis(\pgame))$. However, since any solution $\otherhypothesis^*(\pgame, \hypothesis(\pgame))$ to the inner optimization problem $\max_{\otherhypothesis \in \actionspace^\pgames: \forall \pgame \in \pgames, \otherhypothesis(\pgame) \in \actions(\hypothesis(\pgame))}  \Ex\left[ \cumulregret[][\pgame](\hypothesis(\pgame), \otherhypothesis(\pgame))\right]$ is implicitly parameterized by the choice of equilibrium mapping $\hypothesis$, we can represent this dependence explicitly in the optimization problem, and restrict our selection of $\otherhypothesis$ to a continuously differentiable hypothesis class $\otherhypotheses \subset \actionspace^{\pgames \times \actions}$, and 
% sidestep the issue by obtaining an approximate gradient (that is guaranteed to be bounded) via the implicit function theorem, and in this way
overcome issue (3).

With these observations in mind, given hypothesis classes $\hypotheses \subset \actions[][\pgames]$,
and $\otherhypotheses \subset \actionspace^{\pgames \times \actions}$, the \mydef{generative adversarial learning problem} is to find a tuple $(\hypothesis^*, \otherhypothesis^*) \in \hypotheses \times \otherhypotheses$ that consists  of a \mydef{generator} and \mydef{discriminator} to solve the following optimization problem:
% 
\begin{align}\label{eq:min_max_hypo_abstract}
\!\!    \!\! \min_{\hypothesis \in \hypotheses} \!\!\!\!\max_{\substack{\otherhypothesis \in \otherhypotheses: \forall \pgame \in \pgames,\\ \otherhypothesis(\pgame; \hypothesis(\pgame)) \in \actions[][\pgame](\hypothesis(\pgame))}} \!\!\!\! \Ex_{\pgame \sim \distribpgames} \!\left[ \cumulregret[][\pgame](\hypothesis(\pgame), \!\otherhypothesis(\pgame; \!\hypothesis(\pgame)))\right].
\end{align}
% 
\noindent This problem can be interpreted as a zero-sum game between the generator and the discriminator. The generator takes as input a parametric representation of a pseudo-game, and predicts a solution that consists of an \mydef{action profile}, i.e., a tuple of actions, one per agent. The discriminator  takes the game and the output of the generator as input, and outputs a best-response for each agent (\Cref{fig:network_diagram}). The optimal mappings  $(\hypothesis^*, \otherhypothesis^*)$ for  \Cref{eq:min_max_hypo_abstract} are then called the \mydef{Generative Adversarial Equilibrium Solver (\nees)}.
%\dcp{I think you mean something like ``we refer to the instantiation of the framework to blah the NEEN" (I think of the ``solutions" in this paper as being the equilibria!)}

% Hence, to efficiently compute hypotheses that solve the cumulative regret min-max optimization problem, one needs to assume some hypotheses classes $\hypotheses \subset \actions[][\pgames]$ and $\otherhypotheses \subset \actionspace^{\pgames \times \actions}$, i.e. one needs to restrict the domain of $\hypothesis$ and $\otherhypothesis$

% This explicit representation of the dependence of the inner optimization's solution on the outer hypothesis class selection in turn allows to side step the second issue

% to differentiate the inner optimization problem w.r.t. to the outer hypothesis solution. 

% Note that any solution $\otherhypothesis^*(\pgame, \hypothesis(\pgame))$ to the inner optimization problem $\max_{\otherhypothesis \in \actionspace^\pgames: \forall \pgame \in \pgames, \otherhypothesis(\pgame) \in \actions(\hypothesis(\pgame))}  \Ex\left[ \cumulregret[][\pgame](\hypothesis(\pgame), \otherhypothesis(\pgame))\right]$ is implicitly parametrized by the choice of equilibrium mapping $\hypothesis$. We can choose to represent this dependence explicitly in the optimization problem, that is: 
% \begin{align}
%     % &\min_{\hypothesis \in \actions[][\pgames]} \max_{\otherhypothesis \in \actionspace^{\pgames}: \forall \pgame \in \pgames, \otherhypothesis(\pgame) \in \actions[][\pgame](\hypothesis(\pgame))}  \Ex_{\pgame \sim \distribpgames} \left[ \cumulregret[][\pgame](\hypothesis(\pgame), \otherhypothesis(\pgame))\right]\\ 
%     % &= 
%     \min_{\hypothesis \in \actions[][\pgames]} \max_{\substack{\otherhypothesis \in \actionspace^{\pgames \times \actions}: \forall \pgame \in \pgames,\\ \otherhypothesis(\pgame; \hypothesis(\pgame)) \in \actions[][\pgame](\hypothesis(\pgame))}}  \Ex_{\pgame \sim \distribpgames} \left[ \cumulregret[][\pgame](\hypothesis(\pgame), \otherhypothesis(\pgame; \hypothesis(\pgame)))\right]
% \end{align}


% This explicit representation of the dependence of the inner optimization's solution on the outer hypothesis class selection in turn allows to side step the second issue

% to differentiate the inner optimization problem w.r.t. to the outer hypothesis solution. Unfortunately, the gradient of $
% % \max_{\substack{\otherhypothesis \in \actionspace^{\pgames \times \actions}: \forall \pgame \in \pgames,\\ \otherhypothesis(\pgame; \hypothesis(\pgame)) \in \actions[][\pgame](\hypothesis(\pgame))}}
% \max_{\otherhypothesis}\Ex_{\pgame \sim \distribpgames} \left[ \cumulregret[][\pgame](\hypothesis(\pgame), \otherhypothesis(\pgame; \hypothesis(\pgame)))\right]$ with respect to $\hypothesis$ is quite complicated \emph{even when it exists} due to the constraint $\forall \pgame \in \pgames, \otherhypothesis(\pgame) \in \actions(\hypothesis(\pgame))$ as it involves an integral over $\pgames$. 
% % In fact, without additional assumptions on the hypothesis class, the gradient is not even guaranteed to exist. 
% However, by restricting our selection of $\otherhypothesis$ to a differentiable hypothesis classes $\otherhypotheses \subset \actionspace^{\pgames \times \actions}$ we can sidestep the issue by obtaining an ``approximate'' gradient.
% Hence, to efficiently compute hypotheses that solve the cumulative regret min-max optimization problem, one needs to assume some hypotheses classes $\hypotheses \subset \actions[][\pgames]$ and $\otherhypotheses \subset \actionspace^{\pgames \times \actions}$, i.e. one needs to restrict the domain of $\hypothesis$ and $\otherhypothesis$:
% , i.e., assume a functional form for the hypotheses $\hypothesis$ and $\otherhypothesis$:
% \begin{align}\label{eq:min_max_hypo_abstract}
%     \min_{\hypothesis \in \hypotheses} \max_{\substack{\otherhypothesis \in \otherhypotheses: \forall \pgame \in \pgames,\\ \otherhypothesis(\pgame; \hypothesis(\pgame)) \in \actions(\hypothesis(\pgame))}}  \Ex_{\pgame \sim \distribpgames} \left[ \cumulregret[][\pgame](\hypothesis(\pgame), \otherhypothesis(\pgame; \hypothesis(\pgame)))\right]
% \end{align}


\if 0
That is, the \mydef{Neural Economic Equilibrium Network (\nees{})} is a tuple $(\hypothesis^*, \otherhypothesis^*)$ which corresponds to the solutions of \Cref{eq:min_max_hypo_abstract} that satisfy:
%
\begin{align}
     &\max_{\substack{\otherhypothesis \in \hypotheses: \forall \pgame \in \pgames,\\ \otherhypothesis(\pgame; \hypothesis(\pgame)) \in \actions[][\pgame](\hypothesis(\pgame))}}  \Ex\left[ \cumulregret[][\pgame](\hypothesis^*(\pgame), \otherhypothesis(\pgame; \hypothesis(\pgame)))\right] 
     \notag
     \\ & \leq  \Ex \left[ \cumulregret[][\pgame](\hypothesis^*(\pgame), \otherhypothesis^*(\pgame; \hypothesis(\pgame)))\right] \notag
     \\  &\leq \min_{\hypothesis \in \hypotheses} \max_{\substack{\otherhypothesis \in \otherhypotheses: \forall \pgame \in \pgames,\\ \otherhypothesis(\pgame; \hypothesis(\pgame)) \in \actions[][\pgame](\hypothesis(\pgame))}} \Ex \left[ \cumulregret[][\pgame](\hypothesis(\pgame), \otherhypothesis(\pgame; \hypothesis(\pgame)))\right]
\end{align}
\fi
% \begin{align}
%     \min_{\hypothesis \in \hypotheses} \max_{\otherhypothesis \in \otherhypotheses: \forall \pgame \in \pgames, \otherhypothesis(\pgame; \hypothesis(\pgame)) \in \actions[][\pgame](\hypothesis(\pgame))} \Ex \left[ \cumulregret[][\pgame](\hypothesis(\pgame), \otherhypothesis(\pgame; \hypothesis(\pgame)))\right]
% \end{align}
% The generative adversarial learning problem, can be seen as a two-player min-max (or zero-sum) sequential, i.e., Stackelberg \cite{stackelberg1934marktform}, game between a generator $\hypothesis \in \hypotheses$ and a discriminator $\otherhypothesis \in \otherhypotheses$ such that for each pseudo-game $\pgame \sim \distribpgames$, the generator $\hypothesis$, which corresponds to the equilibrium mapping, first generates an equilibrium guess $\hypothesis(\pgame) \in \actions[][\pgame]$, and then the discriminator $\otherhypothesis$ guesses a best-response profile $\otherhypothesis(\pgame, \hypothesis(\pgame)) \in \actions(\hypothesis(\pgame))$ such that ${\otherhypothesis}_{\player}(\pgame, \hypothesis(\pgame)) \in \actions[\player]({\hypothesis}_{-\player}(\pgame))$ is a best-response to ${\hypothesis}_{-\player}(\pgame)$. After both the generator and discriminator have made their moves the generator (resp. discriminator) incurs a loss (gain) determined by the expected cumulative regret $\Ex\left[ \cumulregret[][\pgame](\hypothesis(\pgame), \otherhypothesis(\pgame; \hypothesis(\pgame)))\right]$. The solutions $\hypothesis^*$ and $\otherhypothesis^*$ then correspond to a Stackelberg equilbrium of the min-max Stackelberg game \cite{goktas2021minmax} given in \Cref{eq:min_max_hypo_abstract}, at which, the generator minimizes its loss assuming that the discriminator best-responses, and the discriminator best-responds.



% learning algorithm which computes a min-max solution of the expected cumulative regret, $\Ex_{\pgame \sim \distribpgames} \left[\cumulregret[][\pgame](\action, \otheraction)\right]$, rather than a minimum of the exploitability. That is, we can re-express the unsupervised equilibrium mapping learning problem as the following generative adversarial learning problem:
% \begin{align}
%     \min_{\hypothesis \in \actions[][\pgames]} \Ex_{\pgame \sim \distribpgames} \left[\exploit[][\pgame](\hypothesis(\pgame)) \right] &= \min_{\hypothesis \in \actions[][\pgames]} \Ex_{\pgame \sim \distribpgames} \left[\max_{\otheraction \in \actions(\hypothesis(\pgame))} \cumulregret[][\pgame](\hypothesis(\pgame), \otheraction)\right]\\ 
%     &= \min_{\hypothesis \in \actions[][\pgames]} \Ex_{\pgame \sim \distribpgames} \left[ \max_{\otherhypothesis[][\pgame] \in \actionspace^\pgames: \otherhypothesis[][\pgame](\pgame) \in \actions[][\pgame](\hypothesis(\pgame))} \cumulregret[][\pgame](\hypothesis(\pgame), \otherhypothesis[][\pgame](\pgame))\right]\\
%     &= \min_{\hypothesis \in \actions[][\pgames]} \max_{\otherhypothesis \in \actionspace^{\pgames}: \forall \pgame \in \pgames, \otherhypothesis(\pgame) \in \actions[][\pgame](\hypothesis(\pgame))}  \Ex_{\pgame \sim \distribpgames} \left[ \cumulregret[][\pgame](\hypothesis(\pgame), \otherhypothesis(\pgame))\right]
% \end{align}


==> Learning Generalized Nash Equilibrium - ICML/prelim.tex <==
\section{Preliminaries}\label{sec:prelim}
% 
% 
% \textbf{Notation.}
\subsection{Notation}
All notation for variable types, e.g., vectors, are clear from context, if any confusions arise see \Cref{sec_ap:prelims}.
%
% We denote functions by a letter determined by the value of the function, e.g., $f$ if the mapping is scalar-valued, $\f$ if the mapping is vector-valued, and $\calF$ if the mapping is set-valued.
%
We denote the set of integers $\left\{0, \hdots, n-1\right\}$ by $[n]$, the set of natural numbers by $\N$, the set of real numbers by $\R$, and the positive and strictly positive elements of a set by a subscript $+$ and $++$, e.g., $\R_+$ and $\R_{++}$.
% subscript, respectively, e.g., $\R_+$ and $\R_{++}$. 
%
% We define the gradient $\grad[\x]: C^1(\calX) \to C^0(\calX) $ as the operator which takes as input a differentiable functional $f: \calX \to \R$, and outputs a vector-valued function consisting of the partial derivatives of $f$ w.r.t. $\x$.
% We denote the orthogonal projection onto a set $C$ by $\project[C]$, i.e., $\project[C](\x) = \argmin_{\y \in C} \left\|\x - \y \right\|_2^2$. 
% We denote the orthogonal projection operator onto a set $C$ by $\project[C]$, i.e., $\project[C](\x) = \argmin_{\y \in C} \left\|\x - \y \right\|^2$. 
We denote by $\simplex[n] = \{\x \in \R_+^n \mid \sum_{i = 1}^n x_i = 1\}$, and by $\simplex(A)$, the set of probability measures on the set $A$.
% We denote the support $\supp(\distribpgames)$ of any probability distribution function $\distribpgames: \pgames \to \R$ is defined as $\supp(\distribpgames) = \{\pgame \in \pgames \mid  \distribpgames(\pgame) > 0 \}$.

% A \mydef{min-max Stackelberg game}, denoted $(\outerset, \innerset, \obj, \constr)$, is a two-player, zero-sum game, where one player, who we call the $\outer$-player (resp.\ the $\inner$-player), is trying to minimize their loss (resp.\ maximize their gain), defined by a continuous \mydef{objective function} $\obj: X \times Y \rightarrow \mathbb{R}$, by choosing a strategy from a compact \mydef{strategy set} $\outerset \subset \R^\outerdim$ (resp. $\innerset \subset \R^\innerdim$) s.t.\ $\constr(\outer, \inner) \geq 0$ where $\constr(\outer, \inner) = \left(\constr[1] (\outer, \inner), \hdots, \constr[\numconstrs](\outer, \inner) \right)^T$ with $\constr[\numconstr]: \outerset \times \innerset \to \R$, for all $\numconstr \in [\numconstrs]$. 
% A strategy profile $(\outer, \inner) \in \outerset \times \innerset$ is said to be \mydef{feasible} iff $\constr[\numconstr] (\outer, \inner) \geq 0$, for all $\numconstr \in [\numconstrs]$.
% The function $\obj$ maps a pair of feasible strategies taken by the players to a real value (i.e., a payoff), which represents the loss (resp.\ the gain) of the $\outer$-player (resp.\ $\inner$-player).
% The relevant solution concept for Stackelberg games is the \mydef{Stackelberg equilibrium (SE)}. A strategy profile $\left(\outer^{*}, \inner^{*} \right) \in \outerset \times \innerset$ s.t.\ $\constr(\outer^{*}, \inner^{*}) \geq \zeros$ is a \mydef{Stackelberg equilibrium} if $\max_{\inner \in \innerset : \constr(\outer^{*}, \inner) \geq 0} \obj \left( \outer^{*}, \inner \right) \leq \obj \left( \outer^{*}, \inner^{*} \right) \leq \min_{\outer \in \outerset} \max_{\inner \in \innerset : \constr(\outer, \inner) \geq 0} \obj \left( \outer, \inner \right)$.
% A min-max game is said to be convex-concave if $\max_{\inner \in \innerset : \constr(\outer, \inner) \geq \zeros} \obj(\outer, \inner)$ is convex in $\outer$, and $\obj(\outer, \inner)$ is concave in $\inner$, for all $\outer \in \outerset$.
%
\subsection{Pseudo-Games}

A \mydef{pseudo-game} \cite{arrow-debreu} $\pgame \doteq (\numplayers, \actionspace,  \actions[][\pgame], \actionconstr[][][\pgame], \util[][][\pgame])$, denoted $(\numplayers, \actionspace,  \actions, \actionconstr, \util)$ when clear from context, comprises $\numplayers \in \N_+$ players, where player $\player \in \players$ chooses an action $\action[\player]$ from a non-empty, compact, and convex \mydef{action space} $\actionspace[\player] \subset \R^\numactions$.
We denote the players' joint action space by $\actionspace = \bigtimes_{\player \in \players} \actionspace[\player] \subset \R^{\numplayers \numactions}$.
Each player $\player \in \players$ aims to maximize their continuous \mydef{payoff},
% \footnote{The assumption that $\util[\player]$ is bounded between 0 and 1 is without loss of generality since the action space is compact, and the utility function is continuous implying that $\util[\player]$ is bounded and its range can thus be normalized to $[0,1]$.}
$\util[\player]: \actionspace \to \R$, which is concave in $\action[\player]$, by choosing a feasible action from a set of actions, $\actions[\player](\naction[\player]) \subseteq \actionspace[\player]$, this depending on the actions $\naction[\player] \in \actionspace[-\player] \subset \R^{(\numplayers-1)\numactions}$ of the other players. Here, $\actions[\player]: \actionspace[-\player] \rightrightarrows  \actionspace[\player]$ is a non-empty, continuous, compact- and convex-valued \mydef{(feasible) action correspondence}. It is this dependence on each others' actions that makes this a pseudo-game, and not just a game.
For convenience, we represent $\actions[\player]$
as $\actions[\player](\naction[\player]) = \{ \action[\player] \in \actionspace[\player] \mid \actionconstr[\player][\numconstr](\action[\player], \naction[\player]) \geq \zeros, \text{ for all } \numconstr \in [\numconstrs]\}$, where for all $\player \in \players$, and $\numconstr \in [\numconstrs]$, $\actionconstr[\player][\numconstr]$ is a continuous and concave function in $\action[\player]$, which defines the constraints.\footnote{This is without loss of generality since any compact convex set can be represented by the superlevel sets of a continuous concave function \cite{rockafellar2009variational}.} 
%
We denote the \mydef{product (feasible) action correspondence} by $\actions(\action) = \bigtimes_{\player \in \players} \actions[\player](\naction[\player])$, which we note is guaranteed to be non-empty, continuous, and compact-valued, but not necessarily convex-valued. We denote $\actions$ the \mydef{set of jointly feasible strategies}, i.e., $\actions = \{\action  \in \actionspace \mid \actionconstr[\player][\numconstr](\action) \geq \zeros, \forall \player \in \players, \numconstr \in [\numconstrs] \}$. We denote the class of all pseudo-games by $\pgames$.\footnote{A \mydef{game} \cite{nash1950existence} is a pseudo-game where, for all players $\player \in \players$, $\actions[\player]$ is a constant correspondence with value $\actionspace[\player]$. A \mydef{normal-form game} is a game where $\actionspace[\player] = \simplex[\numactions]$ and for all $\player \in \players$, $\util[\player]$ is affine.} 

% Given a pseudo-game $\pgame$, an $\varepsilon$-\mydef{generalized Nash equilibrium (GNE)} is strategy profile 
% $\action^* \in \actions(\action^*)$, s.t.~for all $\player \in \players$ and $\action[\player] \in \actions[\player](\naction[\player][][][*])$, $\util[\player](\action^*) \geq \util[\player](\action[\player], \naction[\player][][][*]) - \varepsilon$. 
Given a pseudo-game $\pgame$, a \mydef{generalized Nash equilibrium (GNE)} is strategy profile 
$\action^* \in \actions$, s.t.~for all $\player \in \players$ and $\action[\player] \in \actions[\player](\naction[\player][][][*])$, $\util[\player](\action^*) \geq \util[\player](\action[\player], \naction[\player][][][*])$. 
%
An \mydef{equilibrium mapping}, $\hypothesis: \pgames \to \actions$ is a mapping that takes as input a pseudo-game $\pgame \in \pgames$ and outputs a GNE, $\hypothesis(\pgames)$, for that game. 
% We denote the set of all equilibrium mappings as $\actions[][\pgames]$.

Given a pseudo-game $\pgame$, we define the \mydef{regret} for 
player $\player \in \players$ for  action $\action[\player]$  as compared to another action $\otheraction[\player]$, given the action profile $\action[-\player]$ of other players, as 
%
%\begin{align}
    $\regret[\player][\pgame](\action[\player], \otheraction[\player]; \naction[\player]) = \util[\player][][\pgame](\otheraction[\player], \naction[\player]) - \util[\player][][\pgame](\action[\player], \naction[\player])$.
Additionally, the \mydef{cumulative regret}, $\cumulregret[][\pgame]: \actionspace \times \actionspace \to \R$
between two action profiles $\action \in \actionspace$ and $\otheraction \in \actionspace$
%across all players in a pseudo-game $\pgame \in \pgames$ is 
is given by $\cumulregret(\otheraction; \action) = \sum_{\player \in \players} \regret[\player][\pgame](\action[\player], \otheraction[\player]; \naction[\player])$.
%\enspace .
%\end{align}
%\noindent
% For notational simplicity, we will often write $\regret[\player][\pgame](\action[\player], \naction[\player]) = \max_{\otheraction[\player] \in \actions[\player](\naction[\player][][][*])} \util[\player](\otheraction[\player], \naction[\player]) - \util[\player](\action[\player], \naction[\player])$
Further, the \mydef{exploitability}  (or \mydef{Niakido-Isoda potential  function} \cite{nikaido1955note}),
$\exploit[][\pgame]: \actionspace \to \R$, of an action profile $\action$ is defined as 
$\exploit[][\pgame](\action) =  \sum_{\player \in \players} \max_{\otheraction[\player] \in \actions[\player](\naction[\player])} \regret[\player][\pgame](\action[\player], \otheraction[\player]; \naction[\player])$.
%An alternative name for exploitability in the GNE literature is the Nikaido-Isoda potential function
The max is taken over $\actions[\player](\naction[\player])$,
%to obtain the sum of unilateral deviations, 
since a player can only deviate within the set of feasible strategies. Note that an action profile $\action^*$ is a GNE iff $\exploit[][\pgame](\action^*) = 0$.
% 
% 
% \textbf{Mathematical preliminaries.}
\subsection{Mathematical Preliminaries}
For any function $\obj: \calX \to \calY$, we denote its Lipschitz-continuity constant by $\lipschitz[\obj]$.
For two arbitrary sets $\hypotheses, \hypotheses^\prime \subset \calF$, the set  $\hypotheses^\prime$ \mydef{$\coveringnumber$-covers} $\hypotheses$ (w.r.t. some norm $\| \cdot \|$) if for any $\hypothesis \in \hypotheses$ there exists $\hypothesis^\prime \in \hypotheses^\prime$ such that $\left\|\hypothesis - \hypothesis^\prime \right\| \leq \coveringnumber$. 
The \mydef{$\coveringnumber$-covering number}, $\coveringcard(\hypothesis, \coveringnumber)$, of a set $\hypotheses$ is the cardinality of the smallest set $\hypotheses^\prime \subset \calF$ that $\coveringnumber$-covers $\hypotheses$.
A set $\hypotheses$ is said to have a \mydef{bounded covering number}, if for all $\coveringnumber \in \R_+$, we have that the logarithm of its covering number is polynomially bounded in $1/\coveringnumber$, that is $\log(\coveringcard(\hypothesis, \coveringnumber)) \leq \poly(\nicefrac{1}{\coveringnumber})$. Additional background can be found in \Cref{sec_ap:prelims}.

% Let $\hypothess$ be a vector space over $\R$. A function $\left<\cdot, \cdot\right>_\hypotheses: \hypotheses \times \hypotheses \to \R$ is said to be an \mydef{inner product} if it is \mydef{bilinear}, i.e., $\forall, \alpha_1, \alpha_2 \in \R$ $f_1, f_2, g \in \hypotheses$, $\left<\alpha_1 f_1 + \alpha_2 f_2, g \right>_\hypotheses = \alpha_1 \left<f_1, g \right>_\hypotheses +  \alpha_2 \left< f_2, g \right>_\hypotheses$, \mydef{symmetric}, i.e.,$f, g \in \hypotheses$ $f, g \in \hypotheses$ $\left<f, g \right>_\hypotheses = \left<g, f \right>_\hypotheses$, and \mydef{positive definite}, i.e., $f, g \in \hypotheses$, $\left< f, f \right> \geq 0$ and $\left< f, f \right> = 0 \implies f = 0$.
% A tuple $(\hypotheses, \left<\cdot, \cdot\right>)$ is a \mydef{Hilbert space} if for all $\{f_n\}_{n \in \N_+} \subset \hypotheses$ such that $\sqrt{\left< f_n - f_m, f_n - f_m\right>},  \xrightarrow{\mathrm{unif.}} 0 $, we have that  $\lim_{n \to \infty} f_n = f$ and $f \in \hypotheses$.
% Consider a Hilbert space $(\hypotheses, \left<\cdot, \cdot\right>)$ such that $\hypotheses =  \{f \mid f: \calX \to \R\}$ for $\calX$ non-empty, for all $\x \in  \calX$, the \mydef{(Dirac) evaluation functional} $\dirac[\x]: \hypotheses \to \R$ is given as $\dirac[\x](f) = f(\x)$.
% A Hilbert space $(\hypotheses, \left<\cdot, \cdot\right>)$ is a \mydef{reproducing kernel Hilbert space (RKHS)} if $\dirac[\x](f)$ is continuous for all $\x \in \calX$. 

% The \mydef{projected gradient operator} of a function $f: \actions \to \R$ is defined as
% $\gradmap[{\learnrate[ ][  ]}][{f}](\action) = \action -  \proj[\actions]\left[ \action - \learnrate[\action ][  ] \grad f(\action) \right]$. The projected gradient operator is a special case of the gradient mapping operator, and a generalization of the gradient that is projected back onto the feasible set $\actions$ \cite{beck2017first}.
% The zeros of the projected gradient operator capture stationary points both at the boundary of the set $\actions$ and in its interior.


==> Learning Generalized Nash Equilibrium - ICML/related.tex <==
% \textbf{Additional related work.}
\subsection{Additional Related Work}
We refer the reader to \Cref{sec_app:related} for a survey of methods to compute GNEs, and to \Cref{sec_app:application_motivation} for a survey of applications of GNE. 
%
Our contributions generally relate to a line of work on \emph{differentiable economics}, which seeks to use methods of neural computation for problems of economic design and equilibrium computation.
In regard to finding optimal economic designs, deep learning has been used  for problems of auction design
%
%mechanism can be seen as a neural network from bids to outcomes and trained to maximize a desired objective over a training set of bids %while penalizing failure of incentive compatibility. The mechanisms that have been tackled with this approach include %amongst others %\cite{brero2022learning}\
%revenue-maximizing auctions~
\cite{dutting2019optimal,curry2022learning,tacchetti2019neural,curry2022differentiable, gemp2022designing, rahme2020auction}
and matching~\cite{ravindranath2021deep}.
%
In regard to solving for equilibria, some recent works have tried to solve for Nash equilibria in auctions \cite{heidekruger2019computing, bichler2021learning}, and dynamic stochastic general equilibrium models \cite{curry2022finding, chen2021deep, hill2021solving}. 
% \if 0
% Finally, a related and more theoretical line of work in economics and computer science has aimed to bring tools from machine learning and computational learning theory to design auctions from samples of bidder valuations. Much of the effort here has focused on analyzing the sample complexity of designing revenue-maximizing auctions (see e.g. \cite{cole2014sample, mohri2016learning}). Some works have leveraged machine learning to optimize different aspects of mechanisms (\cite{lahaie2011kernel, dutting2015payment, narasimhan2016automated}).
% This line of work is also closely related to works on automated mechanism design (\cite{conitzer2002complexity, sandholm2015automated}), but these are limited to specialized classes of auctions. The theory we provide in this paper can be placed in light of the developments in these works.
% \fi
% %xx 
% %Our work also extends the use of {\em differentiable economics}~\cite{dutting2019optimal, shen2018automated, curry2022differentiable}, %from mechanism design to general equilibrium theory. 
% %Our framework can be used to solve any pseudo-game, and hence any general equilibrium model, bridging  the gap that has been existing between various general equilibrium models and the associated deep learning methods to solve them.




==> Learning Generalized Nash Equilibrium - ICML/training.tex <==
\section{Convergence and Sample Complexity}\label{sec:theory}

%With the learning problem having been formulated, we now turn our attention to the problem of training, i.e., computing the optimal generator and discriminator.

For training, we propose a stochastic variant of the nested gradient descent ascent algorithm \cite{goktas2021minmax}, which we call \mydef{stochastic exploitability descent}. Our algorithm computes the optimal generator and discriminator  by estimating the gradient of the expected cumulative regret  and exploitability on  a training set  of
pseudo-games. 
% We  provide  convergence and sample complexity bounds.
% 
\begin{algorithm}[!ht]
\caption{Stochastic Exploitability Descent}
\textbf{Inputs:} $\batchpgames, \learnrate[\hypothesis], \learnrate[\otherhypothesis], \numiters[\hypothesis], \numiters[\otherhypothesis],
\weight[][\hypothesis][0],
\weight[][\otherhypothesis][0]$\\
\textbf{Outputs:} $(\weight[][\hypothesis][\iter],
\weight[][\otherhypothesis][\iter])_{\iter = 0}^{\numiters[\hypothesis]}$
\label{alg:cumul_regret}
\begin{algorithmic}[1]
\FOR{$\iter = 0, \hdots, \numiters[\hypothesis] - 1$}
    \STATE Receive batch $\batchpgames[][\iter] \subset \samplepgames$.
    \STATE
    $\weight[][{\hypothesis}][\iter+1] = \weight[][{\hypothesis}][\iter] - \learnrate[\hypothesis][\iter] \left( \nicefrac{1}{\left|\batchpgames[\hypothesis][\iter] \right|}  \sum_{\pgame \in \batchpgames[\hypothesis][\iter]} \left[ \grad[{\weight[][\hypothesis]}] \avg[\cumulregret](\weight[][\hypothesis][\iter], \weight[][\otherhypothesis][\iter]) \right]\right)$
    \STATE $\weight[][\otherhypothesis]  = \zeros$
    \FOR{$s = 0, \hdots, \numiters[\otherhypothesis] - 1$}
        \STATE Receive batch $\batchpgames[][s] \subset \samplepgames$.
            \STATE $\weight[][\otherhypothesis]  =  \weight[][\otherhypothesis] + \learnrate[\hypothesis][s] \left( \nicefrac{1}{\left| \batchpgames[\otherhypothesis][s] \right|}  \sum_{\pgame \in \batchpgames[\otherhypothesis][s]} \grad[{\weight[][\otherhypothesis]}] \avg[\cumulregret](\weight[][\hypothesis][\iter], \weight[][\otherhypothesis]) \right)$
    \ENDFOR
    \STATE $\weight[][\otherhypothesis][\iter + 1] =  \weight[][\otherhypothesis]$
    \ENDFOR
\STATE Return $(\weight[][\hypothesis][\iter],
\weight[][\otherhypothesis][\iter])_{\iter = 0}^{\numiters[\hypothesis]}$
\end{algorithmic}
\end{algorithm}

% \paragraph{Training algorithm.}
\subsection{Training Algorithm}
% 
For purposes of applicability, going forward, we will assume that we have access to the distribution of pseudo-games $\distribpgames$ only indirectly through a \mydef{training set} $\samplepgames \sim \distribpgames$ of $\numsamples \in \N_+$ sampled pseudo-games.
 %
% In practice, one faces two issues: 1) we might not have direct access to the pseudo-game distribution $\pgame$, or it might not be feasible to compute the expectation $\Ex \left[ \cumulregret[][\pgame](\cdot, \cdot))\right] $ in closed form, and 2) it might be impossible to optimize over hypothesis classes $\hypotheses, \otherhypotheses$ directly.
%
% As a result, we  approximate $\Ex_{\pgame \sim \distribpgames} \left[\exploit[][\pgame](\action) \right]$ via the sample mean, $\Ex_{\pgame \sim \mathrm{unif}(\samplepgames)} \left[\exploit[][\pgame](\action) \right] = \frac{1}{\numsamples} \sum_{\pgame \in \samplepgames} \exploit[][\pgame](\action)$ of a \mydef{training set} $\samplepgames \subseteq \pgames$ of $\numsamples \in \N_+$ sampled pseudo-games. 
Additionally, we will assume that the generator $\hypothesis \in \hypotheses$ and discriminator $\otherhypothesis \in \otherhypotheses$ are parameterized by  vectors, $\weight[][\hypothesis], \weight[][\otherhypothesis] \in \R^\numweights$, such that for all pseudo-games $\pgame \in \pgames$, and weight vectors $\weight \in \R^\numweights$, $\hypothesis(\pgame; \weight[][\hypothesis]) \in \actions$ and $\otherhypothesis(\pgame; \hypothesis(\pgame; \weight[][\hypothesis]), \weight[][\otherhypothesis]) \in \actions(\hypothesis(\pgame; \weight[][\hypothesis]))$.

For notational simplicity,  we define the \mydef{expected exploitability} and \mydef{expected cumulative regret}, respectively, as:
\begin{align*}
    &\mean[\cumulregret](\weight[][\hypothesis], \weight[][\otherhypothesis]) = \Ex \left[ \cumulregret[][\pgame](\hypothesis(\pgame; \weight[][\hypothesis]), \otherhypothesis(\pgame, \hypothesis(\pgame; \weight[][\hypothesis]); \weight[][\otherhypothesis]))\right]\\
    &\mean[\exploit](\weight[][\hypothesis]) = \max_{\weight[][\otherhypothesis] \in \R^\numweights: \forall \pgame \in \pgames, \otherhypothesis(\pgame; \weight[][\otherhypothesis]) \in \actions(\hypothesis(\pgame, \weight[][\hypothesis]))} \mean[\cumulregret](\weight[][\hypothesis], \weight[][\otherhypothesis]),
\end{align*}
\noindent
where the expectation is over the distribution of pseudo-games $\pgame \sim \distribpgames$.
%
Similarly, we define the \mydef{empirical cumulative regret} and the \mydef{empirical exploitability} respectively as:
\begin{align*}
    &\avg[\cumulregret](\weight[][\hypothesis], \weight[][\otherhypothesis]) = \Ex \left[ \cumulregret[][\pgame](\hypothesis(\pgame; \weight[][\hypothesis]), \otherhypothesis(\pgame; \hypothesis(\pgame; \weight[][\hypothesis]), \weight[][\otherhypothesis]))\right]\\
    &\avg[\exploit](\weight[][\hypothesis]) = \max_{\weight[][\otherhypothesis] \in \R^\numweights: \forall \pgame \in \pgames, \otherhypothesis(\pgame; \weight[][\otherhypothesis]) \in \actions(\hypothesis(\pgame; \weight[][\hypothesis]))} \avg[\cumulregret](\weight[][\hypothesis], \weight[][\otherhypothesis]),
\end{align*}
\noindent
where the expectation is over the uniform distribution over the training set, $\pgame \sim \mathrm{unif}(\samplepgames)$.
Putting this together, our training problem becomes:
%
\begin{align}
    \min_{\weight[][\hypothesis] \in \R^\numweights} \max_{\substack{\weight[][\otherhypothesis] \in \R^\numweights: \forall \pgame \in \pgames,\\ \otherhypothesis(\pgame; \hypothesis(\pgame; \weight[][\hypothesis]), \weight[][\otherhypothesis]) \in \actions(\hypothesis(\pgame; \weight[][\hypothesis]))}}  \mean[\cumulregret](\weight[][\hypothesis], \weight[][\otherhypothesis]).
    % \Ex_{\pgame \sim \distribpgames} \left[ \cumulregret[][\pgame](\hypothesis(\pgame; \weight[][\hypothesis]), \otherhypothesis(\pgame; \hypothesis(\pgame; \weight[][\hypothesis]), \weight[][\otherhypothesis]))\right]
\end{align}
% \vspace{-1em}
We propose \Cref{alg:cumul_regret} to solve this optimization problem. This is
a nested stochastic gradient descent-ascent algorithm, which for each generator descent step runs multiple stochastic gradient ascent steps on the weights of the discriminator to approximate the empirical cumulative regret by processing the pseudo-games in the training set in \mydef{batches}, i.e., as mutually exclusive subsets of the training set. After the stochastic gradient ascent steps are done, the algorithm then takes a step of stochastic gradient descent on the empirical exploitability w.r.t. the weights of the generator using the discriminator's weights computed by the stochastic gradient ascent steps to compute the gradient. Note that when the hypothesis class of the discriminator is assumed to contain only differentiable functions, the gradient of the generator with respect to its weights exist, and they are given by the implicit function theorem. 

\subsection{Convergence bounds.}
We  give assumptions under which our
algorithm converges to a stationary point of the empirical exploitability in polynomial-time.
%
\begin{assumption}
\label{assum:convergence}
For any player $\player \in \players$ and $\pgame \in \mathrm{supp}(\distribpgames)$:
1.~(Lipschitz-smoothness) their payoff $\util[\player][][\pgame]$ is $\lipschitz[{\grad[\util]}]$-Lipchitz smooth,
2.~(Strong concavity) their payoff $\util[\player][][\pgame]$ is $\scparam$-strongly-concave in $\action[\player]$,
and 3.~(Affinely parameterized hypothesis classes) For all $\hypothesis \in \hypotheses \subset \actions[][\pgames \times \R^\numweights]$, $\otherhypothesis \in \otherhypotheses \subset \actions[][\pgames \times \actions \times \R^\numweights]$, $\pgame \in \pgames$, $\hypothesis(\pgame; \cdot)$, and $\otherhypothesis(\pgame; \cdot)$ are affine. 
\end{assumption}

The following assumption
%, which will be used for the generalization bound and which we present now for notational convenience in the following theorem, is 
is implied by \Cref{assum:convergence}.
%
\begin{assumption}
\label{assum:sample}
(Lipschitz-continuity) For any player $\player \in \players$ and $\pgame \in  \supp(\distribpgames)$, their payoff $\util[\player][][\pgame]$ is $\lipschitz[{\grad[\util]}]$-Lipchitz continuous. 
\end{assumption}

 Lipschitz-smoothness is a standard assumption in the convex optimization literature \cite{boyd2004convex}, while strong concavity in each player's action is an assumption that is much weaker than 
 strong monotonicity of the pseudo-game which is commonly used in the GNE literature to prove convergence results \cite{jordan2022gne}.\footnote{Strong concavity is necessary to obtain our results, since it ensures that the composition of the discriminator and the exploitability satisfy the PL-condition \cite{karimi2016linear} allowing us to obtain convergence to an optimal solution for the discriminator.}
%
 For omitted definitions, and proofs/results we refer the reader to \Cref{sec_ap:prelims} and \Cref{sec_app:proofs} respectively.

 Theorem~\ref{thm:convergence_stationary_approx}
tells us that our algorithm converges to a stationary point of the empirical exploitability at a  $\tilde{O}(\nicefrac{1}{\sqrt{\numiters[\hypothesis]}})$ rate, up to an error term that depends linearly on the distance, $\varepsilon$, of the discriminator computed by the algorithm w.r.t.~to the optimal discriminator.
A smaller $\varepsilon$ results in higher accuracy, at the expense of a longer run time.
%as $\numiters[\otherhypothesis]$ will then increase.
%
\begin{restatable}[Convergence to Stationary Point]{theorem}{thmconvergencestationaryapprox}
\label{thm:convergence_stationary_approx}
Suppose that \Cref{assum:convergence} holds. Let $\singularval[\mathrm{min}](\otherhypothesis)$ be the smallest non-zero singular value of $\otherhypothesis$. If \Cref{alg:cumul_regret} is run with learning rates $\learnrate[\hypothesis][\iter] = \nicefrac{1}{\sqrt{\iter}}$ and $\learnrate[\otherhypothesis][s] = \nicefrac{(2 s + 1)}{(2\singularval[\mathrm{min}](\otherhypothesis)\scparam(s + 1)^2)}$ for all $\iter \in [\numiters[\hypothesis]]$, $s \in [\numiters[\otherhypothesis]]$. Then, for any number of iterations $\numiters[\hypothesis] \in \N_{++}$, and  $\numiters[\otherhypothesis] \geq \frac{\lipschitz[{\grad \avg[\cumulregret]}]^{3} \lipschitz[{\avg[\cumulregret]}]^2 }{2 \singularval[\mathrm{min}](\otherhypothesis)\scparam \varepsilon}$,
the outputs $(\weight[][\hypothesis][\iter])_{t = 0}^{\numiters[\hypothesis]}$
% $(\weight[][\hypothesis][\iter], \weight[][\otherhypothesis][\iter])_{t = 0}^{\numiters[\hypothesis]}$ 
satisfy
%\begin{align}
% $
%     \left( \min_{\iter = 0, \hdots, \numiters[\hypothesis] - 1} \left\|  \grad[{\weight[][\hypothesis]}] \avg[\cumulregret](\weight[][\hypothesis][\iter], \weight[][\otherhypothesis][\iter]) \right\|_2^2 \right)   \leq \frac{ \avg[\exploit](\action[][][0]) -  \avg[\exploit](\action[][][{\numiters[\hypothesis]}])}{\sum_{\iter = 1}^{\numiters[\hypothesis]} \learnrate[\hypothesis ][\iter]}   + \frac{\lipschitz[{\cumulregret \circ  (\hypothesis, \otherhypothesis)}]  \lipschitz[{\grad \avg[\exploit]}]^2}{2} \frac{\sum_{\iter = 1}^{\numiters[\hypothesis]} (\learnrate[\hypothesis ][\iter])^2 }{\sum_{\iter = 1}^{\numiters[\hypothesis]} \learnrate[\hypothesis ][\iter]} + \varepsilon^2  .
% $
%\end{align}
% where $g = \max_{\action \in \actions} \left\|\gradmap[{\learnrate[\action ][  ]}][{\val}](\action[][][]) \right\|_2$
$\left( \min_{\iter = 0, \hdots, \numiters[\hypothesis] - 1} \left\| \grad[\action] \avg[\exploit](\weight[][\hypothesis][\iter]) \right\|_2^2 \right) \in O\left(\frac{\log(\numiters[\hypothesis])}{\sqrt{\numiters[\hypothesis]}} + \varepsilon\right)$ where $\varepsilon > 0$.
% and 
% $\lim\limits_{\numiters[\hypothesis] \to \infty} \left( \min\limits_{\iter \in [\numiters[\hypothesis]]} \left\|  \grad[{\weight[][\hypothesis]}] \avg[\cumulregret](\weight[][\hypothesis][\iter], \weight[][\otherhypothesis][\iter]) \right\|_2^2 \right) = \varepsilon \enspace .$
\end{restatable}



\begin{remark}
This convergence 
%to a stationary point of the empirical exploitability
can be further improved to a convergence to a minimum of the empirical exploitability under stronger assumptions on the pseudo-games that ensure that the empirical exploitability is convex. For instance, for zero-sum, potential, a large class of monotone games,\footnote{We recall that a pseudo-game is said to be \mydef{monotone} (or \mydef{dissipative}) if for all $\action, \otheraction \in \actionspace$
$\sum_{\player \in \players} \left(\grad[{\action[\player]}] \util[\player](\action) - \grad[{\action[\player]}] \util[\player](\otheraction) \right)^T \left( \action - \otheraction \right) \leq 0$.} and a class of bilinear games, 
the empirical exploitability is guaranteed to be convex \cite{flam1994gne}.
\end{remark}

==> comments.tex <==
{\color{blue} David Comments:
Fantastic talk. A few things that came to mind as you presented, in case of use for finalising the paper/future talk:
\begin{enumerate}
    \item Motivation: consider more clearly separating "use for analysis/model" and "use for application" (e.g., cloud) 
    \item In explaining the novelty of GNE to an audience for the first time, I think emphasising simultaneity is important else they think "well, doesn't my action affect your action in chess"?
    \item Another answer to "how can players do this" is that they might find an equil over time (of course it needs the game to be modified in some way such that an action is still well defined if outside of the joint space)
    \item GAN approach is also unsupervised, so you might want a more careful phrasing to distinguish approaches
    \item I always want to know what the input representation of a game is into the G and the D, but that's a detail good to avoid for a talk 
    \item **It's super interesting that this is doing better than 'unsupervised' on Nash games (although I also wondered why you weren't converging... are the results worse than for GNE because action space discrete, making it harder?)
    \item **Given the tatonnement results (and your method doing better), reviewers will definitely need to be convinced you've turned tatonnement as well as possible
    \item For the Scarf result: I also wanted to know how the 'unsupervised' method does
    \item When stating the local optimality convergence result, I think you should say "for an affine G and D"
\end{enumerate}

These notes are from a version of the paper I grabbed yesterday morning.  I hope they help as you push onwards. I'm so impressed that you've already created such a mature draft.
\begin{enumerate}
    \item I would lift up a narrative around the use of "differentiable methods" (i.e., neural nets, deep learning) for economics, including the work of Martin Bichler and work on the design side. I think this is the right way to frame the contribution of this paper. Related to this, on p.2 I think it's important to give more texture on Luke's work and Duan et al, and how they relate to this paper. Also, you should state what, if anything, is known about the use of GANS for game solving, and what is there to take from the Daskalakis 'differential games' work that came up in one of our meetings?

    \item To motivate, it would be helpful if the introduction could give examples of pseudo-games that are not Arrow-Debreu but are more general than regular games. At the moment I think you're non AD examples are all games and not pseudo-games. Also, it would be good, for the uninitiated, to explain whether or not pseudo-games are simultaneous move games, and to emphasize that the action space is continuous and solution concepts do not require randomization (and to state what is known about existence). I think it can also be helpful to explain how PGs generalize regular simultaneous-move games, if indeed they do (i.e., does the action become a mixed strategy in a regular simultaneous move game?). That said, and given how central Arrow-Debreu will be in the paper, it might be a good idea to put a concrete example of an AD set-up in the introduction or preliminaries of the paper in order to explain what a pseudo-game is. I remember that a pseudo-game became clear to me when you explained the dependence of budget sets on prices. (edited) 

    \item The intro, before related work, needs a more extended overview of the algorithm (there should also be a figure showing the generator/discriminator structure somewhere in the paper), the theory you have, and the computational results presented in the paper.

    \item I don't quite understand either Ex 2.1 or Ex 2.2. For Ex 2.1, you have actions in R_+, but do you mean R_{>= 0}? (I think $\R_+$ is strictly larger than zero). Is the intuition for the non-Lipschitz the following: if a2=eps>0 then a1 can be very large and positive and utility to 1 is large and positive. But if a2=0 then utility to 1 is zero? Thus, a1=0 has exploitability zero for a2=0 or large exploitability for a2=eps>0? If this is the idea, it's not coming through clearly at the moment. (By the way, in eq (2), I think it's worth being pedantic and writing b1a2-a1a2+(-a1b2-a1a2)). For Ex 2.2, I don't see the potential for non-Lipschitz exploitability in Eq 8 (also, it's better to format Eqn 6 as b1-a1+(b2-a2)).

    \item In any case, I think you can move the examples and detailed discussion non Liptschitz of exploitability, preventing the straightforward Duan et al. style approach to solving for GNEs, to an appendix. I recommend spending time unpacking the math on p.6 and working hard on explaining (1) why this helps with respect to Lipschitz exploitability, and  (2) why it leads to a GAN formulation. The notation in Eq (10) is problematic because you write $\psi^G$ on an action profile on the LHS and $\psi^G$ on an action profile and some new function f on the RHS. Also, f is not explained before it is used (I think it's the 'defeating action' for each player). The text before Obs 2.3 is also confusing (what does it mean to "compute exploitability "ex post" after having computed expected cumulative regret?) Is Obs 2.3 trivial, with the more important work happening leading up to Eqn 18 and then getting towards Eqn 22? Are you burying the most important part? If so, I think I'd drop the detailed exposition of Obs 2.3 and focus on explaining the more important pieces. I think you need to try to clearly explain (1) what it is, if anything, that makes this Lipschitz (e.g., is it the differentiable hypothesis classes you're referring to leading up to (18)), and then (2) why the formulation you end up with cannot be solved via a standard "flat" unsupervised formulation as in something like bottom p.4., but needs to be solved via a GAN style formulation. In explaining the GAN-style formulation, I wonder if this needs more work. I haven't worked much with GANs, but doesn't the generator they usually just take a random input, and the discriminator a generated output and true output? Your generator seems to take a sampled game as input. Might this need more explanation, e.g., with a figure to map to someones' cartoon understanding of a GAN framework? (Lastly, why is it helpful to talk about Stackelberg formulations in this paper, as you do after Eqn 22? Don't you want to stick with explaining how Eq 22 can be approximately solved via a GAN? I feel getting into Stackelberg discussions can cause confusion over solution concepts. If there's some related work point you want to make, then make it in the related work section. In any case, isn't Alg 1 fixing the follower when taking leader gradients? (Line 3) To me. this looks like Nash not Stackelberg.)
    
    \item Assumption 3.1 needs motivation and discussion. What does this require of the game, and what does this require of the GAN formulation? How practical and well motivated is this? I think you're making assumptions about the neural net architectures that will be quite different from those in your computational work? For Assumption 3.7, it's probably worth reminding that it is non-Lipschitz of exploitability you referred to earlier, not of payoff. (I think Assum 3.7 needs to be moved earlier, since it's used in Lemmas 3.3 and 3.4).
    
    \item  For Section 4.1, should this be compared to Duan et al. or Luke's work? It seems that it would be very useful to show how your GAN approach compares to a direct "learn to minimize exploitability" approach, where that latter approach works. 
    
    \item  I'm worried about the comparison with tatonnement. At the moment it seems it's doing about as well or better than NESS. This needs more discussion. Why is NESS actually better? Also, why do you not include tatonnement in Fig 3, and is it concerning that test is worse than train for NESS? Is there anything that this suggests about your training set-up?

    \item The Kyoto section will want more context, e.g., another paragraph to make it more real and tangible, and probably also a simple numerical example to explain the model. It is important that this application feels very clear and well motivated as a way to anchor the methods in the paper.
\end{enumerate}

Smaller points:
\begin{enumerate}
    \item (p1) I don't get the complexity argument: doesn't it apply equally well to your method, which can be considered an "efficient GNE algorithm". Would it be better just to note this is a worst case complexity result? 
    \item I'd like to see the introduction, and certainly the methods section, speak more directly to how the pseudo-game input is accessed via the learning system; i.e., do you have a representation, or is it accessed through certain kinds of calculations that the generator or discriminator need to be able to do about the game? (edited) 
    \item (p2, top) I find the "not technically a game" language confusing. Are you explaining why pseudo-games are outside the class of regular, simultaneous move games? At the moment you seem to suggest that if one player's action depends on another's then it is not a game, but plenty of sequential move games have this property (chess!).
    \item p.2, para four, this "requires solving a concave maximization problem" needs a citation. Also, I would defer most of the comparative references (e.g., "extends the range of models that we can solve") to the related work, where you can be more specific. At the mo,ent you have to say things like "overwhelming majority".
    \item The related work needs at least one paragraph on neural net/differentiable methods for algorithmic economics, and "nearly all" (top p.3) is not precise enough, and we need more on your [32] paper because it sounds at the moment that it can do a lot and currently undercuts what the reader understands about the contribution in the present paper. Also, it references "first order methods" but you earlier said (mid p.2) that they don't work.
    \item It's feels odd to call this a "classical approach." If so, I'd expect it to have been extensively studied and to have citations! I also don't understand the criticism in regard to needing to generate the entire set of GNE. Why wouldn't I just need to generate one GNE as a prediction target (assuming I know how to break ties across multiple equilibria)?
    \item (top p.5) I don't think you need this comment about the expressiveness of the hypothesis class. An unnecessary detour, perhaps.
\end{enumerate}
That's all for now. Hope it helps!

}

==> figures/figure_intro_model.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}
    % Seller box
    \node (seller) [rectangle, minimum width=2cm, minimum height=1cm] {Seller};
    
    % Firms boxes
    \node (firm1) [rectangle, below of=seller, xshift=-1.5cm, minimum width=2cm, minimum height=1cm] {Firm 1};
    \node (firm2) [rectangle, below of=seller, xshift=1.5cm, minimum width=2cm, minimum height=1cm] {Firm 2};
    
    % Consumers boxes
    \node (consumer1) [rectangle, below of=firm1, xshift=-1.5cm, minimum width=2cm, minimum height=1cm] {Consumer 1};
    \node (consumer2) [rectangle, below of=firm1, xshift=1.5cm, minimum width=2cm, minimum height=1cm] {Consumer 2};
    
    % Prices arrows
    \draw [->] (seller) -- (firm1);
    \draw [->] (seller) -- (firm2);
    \draw [->] (seller) -- (consumer1);
    \draw [->] (seller) -- (consumer2);
    
    % Money arrow
    \draw [->, dashed] (consumer1) -- (firm1);
    \draw [->, dashed] (consumer2) -- (firm2);
    
    \end{tikzpicture}
    \caption{Depiction of the Telecommunication Power Allocation Pseudo-Game.}
    \label{fig:my_label}
\end{figure}

